Orthogonal Gradient Boosting for Simpler Additive Rule Ensembles

Gradient boosting of prediction rules is an efficient approach to learn potentially interpretable yet accurate probabilistic models. However, actual interpretability requires to limit the number and size of the generated rules, and existing boosting variants are not designed for this purpose. Though corrective boosting refits all rule weights in each iteration to minimise prediction risk, the included rule conditions tend to be sub-optimal, because commonly used objective functions fail to anticipate this refitting. Here, we address this issue by a new objective function that measures the angle between the risk gradient vector and the projection of the condition output vector onto the orthogonal complement of the already selected conditions. This approach correctly approximate the ideal update of adding the risk gradient itself to the model and favours the inclusion of more general and thus shorter rules. As we demonstrate using a wide range of prediction tasks, this significantly improves the comprehensibility/accuracy trade-off of the fitted ensemble. Additionally, we show how objective values for related rule conditions can be computed incrementally to avoid any substantial computational overhead of the new method.

==> 2_1_prefix_optimisation.tex <==
% We define the propositions about the $j$th attribute in the data point $\textbf{x}$ with sign $s=\pm 1$ using the $i$th data point as 
% $\cP_j^s=\{\delta(s x_j\geq x_{ij}):1$ $\leq $ $i\leq n\}.$
% Then, we get the set of all propositions about the $j$th attribute as
% $    \cP=\bigcup_{j=1}^{d}\cP_j^{+1}$ $\cup$ $\cP_j^{-1}.$
The candidates evaluated per search node of branch-and-bound have query vectors that are prefixes of an ordered sub-selection of data points, 
because the optimum in objective function is attained or  approximated by a prefix with respect to some presorting order. 
Given a query $q=p_1 \cdots p_l$, the problem is to find a proposition $p$ such that
$
    p=\arg\max_{p\in\cP}\obj(p_1 \cdots p_l p).
    %=\arg\max_{j,s}\arg\max_{p\in\cP_j^s}{\obj(p_1 \cdots p_l p)}.
$
Let an injective map $\sigma:\{1,...,$ $l\}$ $\rightarrow$ $\{1,...,n\}$ be an ordered subsection of $l$ of $n$ data points, such that 
$\sigma(sx_{i,j})$ $\geq$ $\sigma(sx_{i+1,j})$ where $s=\pm 1$ and 
$p_1(x_r)\cdots p_l(x_r)=0$  if $r\notin\text{img}(\sigma)$. 
Then, the \defemph{prefix optimisation problem} is to find $p$ such that
$$
    \max_p{\obj(p_1 \cdots p_l p)}=\max_i{\obj(\sum_{j=1}^i{\textbf{e}_{\sigma(j)}})}.
$$

==> 2_preliminaries_backup.tex <==
% \begin{figure*}[t!]
% % \vskip 0.1in
% \centering
% \includegraphics[width=0.45\columnwidth]{Images/Subspaces.png}
% \hspace{1cm}
% \includegraphics[width=0.45\columnwidth]{Images/orth_demo.png} 
% % \vskip -0.1in
% \caption{
% Illustration of output space for toy regression example with three data points with target values $y_1=-10$, $y_2=-6$, $y_3=5$ and three queries with output vectors $\q_1=(1, 1, 0)$, i.e., $q_1$ selects the first two data points, $\q_2=(0, 0, 1)$, and $\q_3=(0, 1, 1)$. The gradient boosting objective selects $q_1$ with weight $\beta_1=-8$ as first rule, resulting in a negative gradient vector $-\g=(-2, 2, 5)$.
% \emph{Left:} Approximations~\eqref{eq:gen_proj_error} to target subspace (blue) spanned by $\q_1$ and $-\g$. The subspace (green) spanned by $\q_3$ and $\q_1$ is a better approximation than the subspace (orange) spanned by $\q_2$ and $\q_1$.
% However, the latter is selected by standard gradient boosting. %~\eqref{eq:gb_obj}.
% \emph{Right:} After projection onto orthogonal complement of already selected query, angle between $\q_3$ and $-\g$ is smaller than that between $\q_2$ and $-\g$ and is thus successfully selected by orthogonal gradient boosting objective.}
% \label{fig:subspace}
% \end{figure*}
\section{Rule Boosting}\label{grb}

%\subsection{Rule ensembles, risk, and comprehensibility}
An \defemph{additive ensemble} of $k$ rules can be represented by Boolean query functions $q_1, \dots, q_k$ and a \defemph{weight vector} $\weights=(\weight_1, \dots, \weight_k)^T \in \R^k$
that jointly describe a function 
$
    f(\x) = \sum_{i=1}^{k}{\weight_i q_i(\x)}
$,
the output of which can be mapped to the conditional distribution of a target variable $Y | X=\x$.
That is, the queries define the rule antecedents (rule bodies), and the coefficients $\weights$ define the rule consequents, i.e., the output of rule $i$ for input $\x\in \R^d$ is $\weight_i$ if $\x$ satisfies the antecedent, i.e., $q_i(\x)=1$ (and $0$ otherwise).
Moreover, each \defemph{query function} $q_i\from \R^d \to \{0, 1\}$ is a conjunction of $c_i$  \defemph{propositions}, i.e., $q_i(\x)=p_{i,1}(\x)p_{i,2}(\x)\dots p_{i,c_i}(\x)$ where the $p_{i,j}$ are typically a threshold function on an individual input variable, e.g., $p_{i,j}(\x)=\delta(x_l \geq t)$.
We denote the set of available propositions by $\cP$ and the \defemph{query language} of all conjunctions that can be formed from $\cP$ as $\cQ$.
% \begin{equation*}
%     q_i = \bigwedge_{j=1}^{m_i}{p_j}, 
% \end{equation*}


We are concerned with two properties of  additive rule ensembles: (empirical) regularised \defemph{risk}
%\footnote{While $l_2$-regularization can be added to all algorithms, we focus on the unregularized case for ease of exposition.}
$
    R(f) = \frac{1}{n}\sum_{i=1}^{n}{l(f(\x_i), y_i)} + \lambda \|\weights\|^2/n
$,
measured by some positive loss function $l(f(\x), y)$ averaged over a dataset $\{(\x_1, y_1),\dots, (\x_n, y_n)\}$,
and \defemph{complexity} $C(f) = k + \sum_{i=1}^k c_i$, approximating the cognitive effort required to parse all rule consequents and antecedents.
Here we consider loss functions that can be derived as negative log likelihood (or rather deviance function) when interpreting the rule ensemble output as natural parameter of an exponential family model of the target variable, which  guarantees that the loss function is strictly convex and twice differentiable.
%This has several advantages. Firstly, the resulting rule ensembles can be interpreted as probabilistic models that encode a conditional distribution $Y | X=x$. Hence, besides enabling predictions via $E[Y| X=x]$, they also provide calibrated uncertainty estimates.
%Moreover, it also guarantees that the loss function is strictly convex and twice differentiable. 
Specifically, we consider the cases of \defemph{squared loss} $l_\mathrm{sqr}(f(x_i), y_i) = (f(x_i)-y_i)^2$, the \defemph{logistic loss} $l_\mathrm{log}(f(x_i), y_i)=\log(1+\exp(-y_if(x_i)))$, and the \defemph{Poisson loss} $l_\mathrm{poi}(f(x_i), y_i)=y_i\log y_i-y_if(x_i)-y_i+\exp(f(x_i))$.
\begin{comment}
Specifically, we consider the cases of \defemph{squared loss} 
\begin{equation*}
l_\mathrm{sqr}(f(x_i), y_i) = (f(x_i)-y_i)^2
\end{equation*}
for regression problems where we model $Y | x$ as normally distributed with mean $f(x)$, \defemph{logistic loss} 
\begin{equation*}
l_\mathrm{log}(f(x_i), y_i)=\log(1+\exp(-y_if(x_i)))
\end{equation*}
for (binary) classification where we model $Y| x$ as Bernoulli distributed with positive probability $1/(1+\exp(-f(x)))$ and \defemph{Poisson loss} 
\begin{equation*}
l_\mathrm{poi}(f(x_i), y_i)=\log y_i-f(x_i)-y_i+\exp(f(x_i))
\end{equation*}
for count regression where we model $Y | x$ as Poisson distributed with mean $\exp(f(x))$.
\end{comment}

\paragraph{Gradient boosting}
Gradient boosting~\citep{friedman2001greedy} is a ``stagewise'' fitting scheme for additive models that, in our context, produces a sequence of rule ensembles $f^{(0)}, f^{(1)}, \dots, f^{(k)}$ such that $f^{(0)}(\x)= 0$ and, for $t \in [1, k]$, $f^{(t)}(\x)=f^{(t-1)}(\x)+\weight_t q_t(\x)$. 
%In other words, it is a greedy approach that fits one rule per iteration without correcting the previously fitted rules.
%Specifically, the seminal idea in \citet{friedman2001greedy} is to choose the query (or ``baselearner'') in iteration $t$ to perform an approximate gradient descent in $\R^n$---the model ``output space'' defined by the  training data. 
Specifically, the term $\weight_t q_t(\x)$ is chosen to perform an approximate gradient descent with respect to the risk function $R(f)=R(\f)$ considered as a function of the model \defemph{output vector} $\f=(f(\x_1),\dots, f(\x_n))$.
% This gradient $\g$ has components $g_i=\partial l(f(x_1), y_1) / \partial f(x_i)$
% a current model function $f$, we define the \defemph{gradient vector} as 
% \begin{equation}
%     \g = \left(\frac{\partial l(f(x_1), y_1)}{\partial f(x_1)}, \dots, \frac{\partial l(f(x_n), y_n)}{\partial f(x_n)}\right)^T
%     \label{eq:grad_vector}
% \end{equation}
% $\g=\nabla_{f(\textbf{x})}{R(f)}$
The exact gradient descent update would be $-\alpha_*\g$ where $\g$ is the \defemph{gradient vector} with components $g_i=\partial l(f(\x_i), y_i) / \partial f(\x_i)$ and $\alpha_*$ is the step length that minimizes the empicical risk $R(\f-\alpha\g)$.
%Here we consider $R(f)=R(\f)$ as a function of the model output and identify $f$ with its \defemph{output vector} $\f=(f(x_1),\dots, f(x_n))$.
However, since in general there is no query $q$ for which the output vector $\q=(q(x_1),\dots, q(x_n))$ is equal to the gradient $\g$, the goal is to select $\q^*$ that best approximates $\g$ in the sense that it minimizes the squared \defemph{projection error}
\begin{equation}
    \min_{\beta \in \R} \|-\!\alpha_* \g - \beta \q \|^2 = \alpha_*^2\left(\|\g\|^2 - \frac{(\inner{\q}{\g})^2}{\|\q\|^2}\right) \enspace .
    \label{eq:1d_proj_error}
\end{equation}
This is achieved by choosing $q_t$ to maximize the standard \defemph{gradient boosting objective}~\citep{dembczynski2010ender} $\gbobj(q)=|\inner{\q}{\g}| / \|\q\|$ and to find $\beta_{t} = \argmin_{\beta \in \R} R(\f + \beta\q_t)$ via a line search.
% Therefore, a direct implementation of gradient boosting for rule ensembles is achieved by the following updates that are used in~\citet{dembczynski2010ender}:
% \begin{align}
%     q_{t} = \argmax_{q \in \cQ} \underbrace{|\inner{\q}{\g}| / \|\q\|}_{\gbobj(q)}
%     \text{, }
%     \beta_{t} = \argmin_{\beta \in \R} R(\f + \beta\q_t) % \label{eq:gb_obj}
% \end{align}
% That is, the \defemph{gradient boosting objective} for query selection is to maximize the cosine (or minimize the angle) of the query output vector and the gradient vector.
Note that this $\beta_t$ is not generally equal to the minimizing $\beta$ in~\eqref{eq:1d_proj_error}, because the optimal update in direction $\q$ can be better than the best geometric approximation to the gradient descent update in direction $\q$.
A derivation of this objective function is the \defemph{gradient sum objective}~\citep{dembczynski2010ender, shalev2010trading} $\gsobj(q)=|\inner{\q}{\g}|$, 
which always selects more general rules than the gradient boosting objective~\citep[Thm.~1]{dembczynski2010ender}, however,  typically at the expense of an increased risk per rule, because the correction of data points with large gradient elements has to be toned down to avoid over-correction of other selected data points with small gradient elements.
Finally, an adaption of ``extreme gradient boosting''~\citep{chen2016xgboost} to rule ensembles yields the \defemph{extreme boosting objective}~\citep{boley2021better} $\xgbobj(q)=(\inner{\q}{\g})^2 / \inner{\q}{\h}$ 
where $\h=\text{diag}(\nabla^2_{f(\textbf{x})}{R(f)})$ is the diagonal vector of the risk Hessian  again with respect to the output vector $\f$.
This approach starts from the second order approximation of $R(\f + \beta\q)$ for which also yields a closed form weight update $\beta_{t} = -\inner{\q}{\g}/\inner{\q}{\h}$.
This approach is well-defined for our loss functions derived from exponential family response models, which guarantee defined and positive $\h$.
For the squared loss, it is equivalent to standard gradient boosting, because the second order approximation is exact for $l_\mathrm{sqr}$ and $\h$ is constant.
%A derivation of these updates discussed in both~\citet{dembczynski2010ender} and~\citet{shalev2010trading} is to drop the normalization $\|\q\|$ and instead use only the sum of selected gradient elements, i.e.,
% \begin{equation}
%     q_{t} = \argmax_{q \in \cQ} \underbrace{|\inner{\q}{\g}|}_{\gsobj(q)}\label{eq:gs_obj}
% \end{equation}
% which we refer to here as \defemph{gradient sum objective}.
% This variant always selects more general rules than the gradient boosting objective~\citep[Thm.~1]{dembczynski2010ender}, however,  typically at the expense of an increased risk per rule, because the correction of data points with large gradient elements has to be toned down to avoid over-correction of other selected data points with small gradient elements.

% A further variant of the original gradient boosting approach is ``extreme gradient boosting''~\cite{chen2016xgboost}, which is the basis of the additive rule ensemble algorithm presented in~\citet{boley2021better}. This approach starts from the second order approximation of $R(\f + \beta\q)$ for which the closed form solution yields the \defemph{extreme boosting objective} function and closed form weight updates
% \begin{align}
%     q_{t} = \argmax_{q \in \cQ} \underbrace{(\inner{\q}{\g})^2 / \inner{\q}{\h}}_{\xgbobj(q)}\text{, }
%     \beta_{t} = -\inner{\q}{\g}/\inner{\q}{\h} \label{eq:xgb_obj}
% \end{align}
% where $\h=\text{diag}(\nabla^2_{f(\textbf{x})}{R(f)})$ is the diagonal vector of the risk Hessian matrix again with respect to the output vector $\f$.
% \begin{equation*}
%     \h = \left(\frac{\partial^2 l(f(x_1), y_1)}{\partial f(x_1)^2}, \dots, \frac{\partial^2 l(f(x_1), y_1)}{\partial f(x_n)^2}\right)^T \enspace .
% \end{equation*}
%This approach is well-defined for our loss functions derived from exponential family response models, which, as mentioned above, guarantee that $\h$ is defined and has only positive components.
%Moreover, for the squared loss, the extreme boosting objective is equivalent to standard gradient boosting, because the second order approximation is exact for $l_\mathrm{sqr}$ and $\h$ is constant.
%the updates defined by~\eqref{eq:xgb_obj} are equivalent to those given by~\eqref{eq:gb_obj}

\paragraph{Single rule optimization}
%weight update can be done by Newton search
%remains: how to find query
%last decades ML literature: greedy optimization, designed for classification and regression trees for efficient generation of hundreds of trees (and thousands of rules)
%however, we are interested in small number of rules
%problem: misses the very interactions that are the reason why we prefer rule ensembles over simpler additive models like generalized linear models and generalized additive models
While the rule optimization literature can be  divided into exact branch-and-bound and heuristic (greedy / beam) search, these approaches are actually closely related: they can both be described as traversing a lattice on the query language $\cQ$ imposed by a \defemph{specialization relation} $q \gen q'$ that holds if the propositions in $q'$ are a superset of those mentioned in $q$, and $q'$ thus logically implies $q$.
The difference between the approaches is how they generate and discard specializations of candidate queries.

Here, we build on the branch-and-bound framework presented in~\citet{boley2021better} that allows to efficiently search for optimal conjunctive queries in a condensed search space, given that there is an admissible, effective, and efficiently computable bounding function for the employed objective.
Specifically, let $\obj\from \cQ \to \R$ denote the objective function to be maximized. Then a \defemph{bounding function} $\bnd\from \cQ \to \R$ is  \defemph{admissible} if for all $q \in \cQ$ it holds that $\bnd(q) \geq \best(q)$ where 
% \begin{equation*}
$
    \best(q) = \max_{q \gen q' \in \cQ} \obj(q')
$
% \end{equation*}
denotes the objective value of the best specialization of $q$. A bounding function is effective in allowing to prune the search space if the difference $\bnd(q)-\best(q)$ tends to be small, rendering $\best(q)$ itself the theoretically most effective bounding function.
However, computing $\best(q)$ is as hard as the overall optimization problem.

A frequently applied recipe for constructing an admissible bounding function that is also effective and efficiently computable is to relax the quantifier in the definition of $\best$ and instead of bounding the value of the best specialization in the search space, bound the value of the best subset of data points of those selected by $q$~\citep{morishita2000transversing}. This results in the \defemph{ selectability relaxed} bounding function 
\begin{equation}
\bnd(q) = \max\{\obj(\q'): \q' \leq \q, \q' \in \{0, 1\}^n\}\label{eq:tight_bound}
\geq \best(q) \enspace .
\end{equation}
Here, $\q \leq \q'$ refers to the component-wise less or equals relation on the binary output vector of $q$ and $q'$.
This function can be efficiently computed for many objective functions by pre-sorting the data in time $O(n \log n)$ that has to be carried out only once per fitted rule~\citep{lemmerich2016fast}. 
For instance for the extreme boosting objective, the optimum $q' \in \{0, 1\}^n$ can be found as a prefix or suffix of all data points after sorting them according to the ratio $g_i/h_i$ of first and second order loss derivatives.

%extreme ends: rulefit has very bad comprehensibility; other end recent approaches that fully optimize.
%inbetween: boosting-based approaches
%in this work we consesquently follow through with all choices required to fit rule ensembles for interpretability: full weight correction and optimal fitting

% \begin{equation*}
%     \f = [\q_1, \dots, \q_k]\weights
% \end{equation*}



%Old
%------------------
% \section{Gradient rule boosting}\label{grb}

% An additive rule ensemble can be represented as
% \begin{equation*}
%     f(x) = \sum_{i=1}^{k}{w_i q_i(x)}=\textbf{w}\cdot\textbf{q}(x),
% \end{equation*}
% where $q_i$ is a conjunction of $m_i$ boolean propositions:
% \begin{equation*}
%     q_i = \bigwedge_{j=1}^{m_i}{p_j}, 
% \end{equation*}
% and therefore, it is a boolean function as well.

% To learn an additive rule ensemble, given a set of training data $\{(x_i, y_i)\}_{i=1}^{n}$ which is drawn from the joint distribution of feature variables $X\in\mathbb{X}$ and output variable $Y\in\mathbb{Y}$, the goal is to find an additive rule ensemble with a number of components which minimises the risk function:
% \begin{equation*}
%     R(f) = \mathbb{E}_{X, Y}l(f(x_i), y_i),
% \end{equation*}
% where $l$ is a loss function. 
% The loss function measures the cost if the model output is $f(x)$ when the actual output is $y$, for example, squared loss $l(f(x_i), y_i) = (f(x_i)-y_i)^2$ is usually used for regression problems, logistic loss $l(f(x_i), y_i)=\log(1+\exp(-y_if(x_i)))$ is usually used for classification problems, and Poisson loss $l(f(x_i), y_i)=\log y_i-f(x_i)-y_i+\exp(f(x_i))$ is used for Poisson regression problems for counting outputs.

% However, usually the joint distribution of $X$ and $Y$ is unknown, so we use empirical risk instead:
% \begin{equation}
%     \hat{R}(f) = \frac{1}{n}\sum_{i=1}^{n}{l(f(x_i), y_i)}.
% \end{equation}

% Each iteration of boosting can be done in two steps: query selection and weight calculation. In the first step, a query is selected based on some objective functions. 
% After a query is chosen, we can calculate the weight of the query in a normal boosting framework, or we can also recalculate the weights of all existing queries in the rule ensemble.

% Gradient boosting is firstly introduced by \citet{friedman2001greedy}. 
% In each of its iterations, gradient boosting finds a query which satisfies:
% \begin{equation}\label{eq:gb_goal}
%     \min_\alpha {\norm{\alpha \textbf{q}^*-\textbf{g}}^2}=\min_{\alpha, \textbf{q}} {\norm{\alpha \textbf{q}-\textbf{g}}^2},
% \end{equation}
% where $\textbf{g}=\nabla \hat{R}(f)$ is the gradient vector of the current empirical risk in terms of the model's output. Equation \eqref{eq:gb_goal} yields the objective function of gradient boosting:
% \begin{equation}\label{eq:gb_obj}
%     \text{obj}_\text{gb}=\frac{|\textbf{q}\cdot\textbf{g}|}{\norm{\textbf{q}}},
% \end{equation}
% and this objective function should be maximised.

% If there is a vector $w^*_g\textbf{g}\in\text{span}\{\textbf{g}\}$, then \eqref{eq:gb_goal} finds the $\textbf{q}$ which minimises the distance between $w^*_g\textbf{g}$ and the subspace spanned by $\textbf{q}$. 
% Therefore, gradient boosting selects the base learner (query) which leads to the best geometric approximation of ensemble which adds $\textbf{g}$ with a risk-minimising weight.
% \begin{proposition}
% Gradient boosting identifies the 1d subspace spanned by a query $\textbf{q}$ which approximates best to the 1d subspace spanned by $\textbf{g}$.
% \end{proposition}


==> 3_main_contributions.tex <==
\section{Improved Risk Reduction per Rule}\label{fcogb}
\begin{figure}[t!]
% \vskip 0.1in
\centering
\includegraphics[width=0.47\columnwidth]{Images/Subspace3.png}
% \hspace{0.2cm}
\includegraphics[width=0.47\columnwidth]{Images/orth_demo5.png} 
\vskip -0.1in
\caption{
Output space of  regression example with three data points with target values $\y=(-10, -6, 5)$ and three queries with outputs $\q_1=(1, 1, 0)$, i.e., $q_1$ selects the first two data points, $\q_2=(0, 0, 1)$, and $\q_3=(0, 1, 1)$. Gradient boosting  selects $q_1$ with weight $\beta_1=-8$ as first rule, resulting in negative gradient  $-\g=(-2, 2, 5)$.
\emph{Left:} Approximations~\eqref{eq:gen_proj_error} to target subspace (blue) spanned by $\q_1$ and $-\g$. The subspace (green) spanned by $\q_3$ and $\q_1$ is a better approximation than the subspace (orange) selected by standard gradient boosting (spanned by $\q_2$ and $\q_1$). %~\eqref{eq:gb_obj}.
\emph{Right:} After projection onto orthogonal complement of already selected query, angle between $\q_3$ and $-\g$ is smaller than that between $\q_2$ and $-\g$ and is thus successfully selected by orthogonal gradient boosting objective.}
\label{fig:subspace}
\end{figure}
%In this section, we firstly show the variant to boosting algorithm which recalculate all weights of existing rules in the generated ensemble, i.e. fully-corrective boosting. The objective function of gradient boosting cannot find the best approximation to the subspace spanned by existing queries and gradient in fully-corrective boosting. Therefore, we derive a novel objective function which takes the weight-correction step into consideration during the selection of queries. 

Having reviewed the existing rule boosting approaches, we now turn to improving them in terms of their risk/complexity trade-off.
Our approach to this is to improve the risk reduction per rule added to the ensemble, which directly affects the number of rules needed to achieve a certain risk. 
As it turns out, this typically coincides with preferring the addition of more general and hence simpler rules, hence also positively affects the complexity on the level of rule lengths.

% \begin{figure}[tbh]
% \vskip 0.1in
% \centering
% \includegraphics[width=\columnwidth]{Images/orth_demo.png} 
% \caption{Illustration of orthogonal gradient boosting for a toy scenario with three data points (values marked with blue dots) corresponding to a three-dimensional output space: The negative risk gradient ($-g$, black) lies in the plane (highlighted in light blue) orthogonal to the already selected rule $w_1q_1$, which covers data points $x_1$ and $x_2$. For the second rule, the first candidate query ($q_2$, in orthogonal plane) covers only $x_3$ and is preferred by standard gradient boosting. The second candidate query ($q_3$) is more general, covering $x_2$ and $x_3$, but has a larger projection error initially. However, after orthogonalization ($q'_3$) it is preferred by orthogonal gradient boosting.}
% % output space for three datapoints 
% % already selected rule with query
% % gradient
% % two candidate queries for second rule
% % one (q1, already orthogonal to selected query) is closer to gradient and preferred by standard boosting
% % second (q2) is further away from gradient but closer after projection (dashed lione
% \label{fig:orth_demo}
% \vskip -0.1in
% \end{figure}

% \begin{figure*}[tbh]
% \vskip 0.1in
% \centering
% \includegraphics[width=\columnwidth]{Images/Subspaces.png}
% \includegraphics[width=\columnwidth]{Images/orth_demo.png} 
% \caption{
% Illustration of output space for toy regression example with three data points with target values $y_1=-10$, $y_2=-6$, $y_3=5$ and three queries with output vectors $\q_1=(1, 1, 0)$, i.e., $q_1$ selects the first two data points, $\q_2=(0, 0, 1)$, and $\q_3=(0, 1, 1)$. The gradient boosting objective selects $q_1$ with weight $\beta_1=-8$ as first rule, resulting in a negative gradient vector $-\g=(-2, 2, 5)$.
% \emph{Left:} Approximations~\eqref{eq:gen_proj_error} to target subspace (blue) spanned by $\q_1$ and $-\g$. The subspace (green) spanned by $\q_3$ and $\q_1$ is a better approximation than the subspace (orange) spanned by $\q_2$ and $\q_1$.
% However, the latter is selected by standard gradient boosting~\eqref{eq:gb_obj}.
% \emph{Right:} After projection onto orthogonal complement of already selected query, angle between $\q_3$ and $-\g$ is smaller than that between $\q_2$ and $-\g$ and is thus successfully selected by orthogonal gradient boosting objective.}
% \label{fig:subspace}
% \end{figure*}
\subsection{Weight Correction}
A natural idea to reduce the ensemble risk per rule added is to relax the strict stagewise fitting of traditional gradient boosting and to allow the whole weight vector $\weights$ to be adjusted in every round $t$, i.e., to set
\begin{equation}
    \weights^{(t)} = \argmin_{\beta \in \R^t} R(\Q_t\weights) \enspace ,
    \label{eq:weight_correction}
\end{equation}
where $\Q_t=[\q_1, \dots, \q_t]$ is the $n\times t$ \defemph{query matrix} with the output vectors of all selected queries as columns.
In contrast to a full joint optimization of queries and weights, this intermediate solution still retains the computational benefits of gradient boosting for small rule ensembles:
Given that our loss function $l$ and therefore the empirical risk $R$ are convex, optimizing the weights in round $t$ is a convex optimization problem in $t$ variables, equivalent to fitting a small generalized linear model.
Using Newton-Raphson (``iterated least squares'') type algorithms, the computational cost of this is usually negligible compared to the more expensive query optimization step.
%, especially when aiming for optimal individual queries for their reduced cognitive complexity.

Re-optimizing the weights, which is sometimes referred to as \defemph{fully corrective boosting}~\citep{shalev2010trading}, effectively turns boosting into a form of forward variable selection for linear models.
However, in contrast to conventional variable selection where all variables are given explicitly, we still have to identify a good query $q_t$ in each boosting iteration, 
and it turns out that finding the appropriate query is more complicated as in the case of single weight optimization characterized by~\eqref{eq:1d_proj_error}.
We still would like to add the direction of steepest descent, i.e., the negative gradient $-\g$, to the subsequent risk optimization step and approximate as closely as possible the outcome $[\Q_{t-1}; \g]\boldsymbol{\alpha}^*$ where $\alphavec^* \in \R^t$ are the risk minimizing weights for $\q_1, \dots, \q_{t-1}, \g$.
Therefore, the best approximating query $q$ is now given by
\begin{equation}
    \argmin_{q \in \cQ} \min_{\weights \in \R^t} \| [\Q_{t-1}; \g]\boldsymbol{\alpha}^* - [\Q_{t-1}; \q]\weights\|^2
    \label{eq:gen_proj_error} \enspace .
\end{equation}
Importantly, the standard gradient boosting objective does not generally identify the optimally approximating query, as demonstrated by the example in Fig.~\ref{fig:subspace}: $\spanof\{\q_1, \q_3\}$ (green), is a better approximation to $\spanof\{\q_1, -\g\}$ (blue) than  $\spanof\{\q_1, \q_2\}$ (orange). However, the latter is selected by standard gradient boosting, because the angle between $\q_2$ and $-\g$ is smaller than that between $\q_3$ and $-\g$.

% Traditionally, boosting algorithms generates weak learners in each iteration, but the generated weak learners are not changed in the following iterations.
% However, in the context of rule ensemble learning, if the weights of a query is not changed, once the data points covered by this query are also covered by other queries generated later, the original weights cannot be optimal any more, although they are optimal when they are calculated.
% Therefore, to get a more accurate rule ensemble, we consider reweighting all the queries after a query is selected.

% To reweigh all the queries, we find a weight vector $\weights \in \R^t$ to minimize the empirical risk over $ \text{span}\{\textbf{q}_1,\cdots,\textbf{q}_t\}$, i.e.,
% \begin{equation}
%     \weights_t = \argmin_{\weights \in \R^t} R(\Q_t\weights)
%     \label{eq:weight_correction}
% \end{equation}
% where $\Q_t=[\q_1, \dots, \q_t]$ is the $n\times t$ \defemph{query matrix} with the output vectors of all selected queries as columns.
% \begin{equation}
%     \hat{R}(\textbf{w}^*)=\min_{\textbf{w}}{\hat{R}(\textbf{w})}.
% \end{equation}
% Given that our loss function $l$ and therefore the empirical risk $R$ are convex, solving this optimization problem is inexpensive relative to the overall computational complexity of the gradient boosting algorithm (especially when solving the single query optimization problem optimally via branch-and-bound). 
% In fact, the problem is equivalent to fitting one generalized linear model with $t$ input variables, which can be efficiently solved, e.g., with the Newton-Raphson algorithm (also referred to as \emph{iterated least squares} in this context).

% To get the minimum value of the empirical training risk, we can solve the equation
% \begin{equation}\label{eq:find_w}
%     \frac{\partial \hat{R}(\textbf{w})}{\partial \textbf{w}}=0.
% \end{equation}
% Here, Newton's method or Gradient descent method can be used to solve \eqref{eq:find_w}.


\subsection{Best Subspace Approximation}

The intuitive reason for the gradient boosting objective failing to identify the correct query in Fig.~\ref{fig:subspace} is that selecting $x_2$ in addition to $x_3$ is not beneficial for the overall risk reduction \emph{if} we are only allowed to set the weight for the newly selected query. 
This is because then this weight has to be a compromise between the two different magnitudes of correction required for $x_2$, which only needs a small positive correction, and $x_3$, which needs a large positive correction.
If we, however, are allowed to change the weight of the previously selected query this consideration changes, because we can now balance an over-correction for $x_2$ by adjusting the weight of the first rule.
While on first glance it seems unclear how much of such re-balancing can be applied without harming the overall risk,
it turns out that this is captured by a simple criterion based on the norm of the part of the newly selected query that is orthogonal to the already selected ones (see SI~\citep{github_url} for all proofs).
\begin{lemma}\label{th:objective_func}
    For $\g\! \in \!\R^n$, $\Q\!=\![\q_1, \dots, \q_{t-1}] \in \R^{n \times (t-1)}$, and $\f\! \in \! \spanof\{\q_1, \dots, \q_{t-1}, \g\}$, we have
    \begin{equation}
        \argmin_{q \in \cQ} \min_{\weights \in \R^t} \|\f - [\q_1, \dots, \q_{t-1}, \q]\weights\|^2 = \argmax_{q \in \cQ} \frac{|\inner{\g_\perp}{\q}|}{\|\q_\perp\|} \enspace .
    \end{equation}
    where for a vector $\vecv \in \R^n$ we denote by $\vecv_\perp$ its projection onto the orthogonal complement of $\range \, \Q$.
\end{lemma}
% \begin{proof}
%     Let $\f=[\Q; \g]\alpha$ and $\tilde{\f}=[\Q; q]\weights$. We can decompose the squared error
%     \begin{align*}
%         \|\f-\tilde{\f}\|^2 &= \|[\Q; \g]\alphavec - [\Q; \q]\weights\|^2\\
%         &=\|[\Q; \g_\parallel + \g_\perp]\alphavec - [\Q; \q_\parallel + \q_\perp]\weights\|^2\\
%         &=\|[\Q; \g_\parallel]\alphavec + \alpha_t\g_\perp - [\Q; \q_\parallel]\weights + \weight_t\q_\perp \|^2\\
%         &=\|[\Q; \g_\parallel]\alphavec - [\Q; \q_\parallel]\weights\|^2 + \|\alpha_t \g_\perp - \beta_t \q_\perp\|^2
%     \end{align*}
%     where the last step follows from the Pythagorean theorem and the fact that $\alpha_t \g_\perp - \beta_t \q_\perp$ is an element from the orthogonal complement of $\range [\Q; \g_\parallel]=\range[\Q; g_\parallel]=\range\, \Q$.
%     The equality of these ranges also implies that $\beta_1, \dots, \beta_{t-1}$ can, for all choices of $\beta_t$, be chosen such that the left term of the error decomposition is $0$. Setting $\gamma=\beta_t/\alpha_t$, it follows that
%     \begin{align*}
%         \min_{\weights \in \R^t} \|\f-\tilde{\f}\|^2 &= \min_{\beta \in \R^t} \|\alpha_t \g_\perp - \beta_t \h_\perp\|^2\\
%         &=\min_{\gamma \in \R^t} \alpha^2_t \|\g_\perp - \gamma \q_\perp\|^2\\
%         &=\min_{\gamma \in \R^t} \alpha_t^2 (\|\g_\perp\|^2-2\gamma \inner{\q_\perp}{\g_\perp} + \gamma^2\|\q_\perp\|^2) \\
%         \intertext{and plugging in the minimizing $\gamma=\inner{\q_\perp}{\g_\perp}/\|\q_\perp\|^2$ }
%         &=\alpha^2(\|\g_\perp\| - (\inner{\g_\perp}{\q_\perp})^2/\|\q_\perp\|^2) \enspace ,
%     \end{align*}
%     from which, noting that $\inner{\g_\perp}{\q_\perp}=\inner{\g_\perp}{\q}$, the claim follows.
% \end{proof}
From this result we can directly derive $|\inner{\g_\perp}{\q}|/\|\q_\perp\|$ as suitable objective function for fully corrective gradient boosting.
However, it is worth incorporating two further observations. 
Firstly, we can show that, after applying the weight correction step~\eqref{eq:weight_correction}, the gradient vector satisfies $\g=\g_\perp$, i.e., it is orthogonal to the subspace spanned by the selected queries, and therefore can be used in the objective function without projection.
\begin{lemma}
Let $\g$ be the gradient vector after the application of the weight correction step~\eqref{eq:weight_correction} for selected queries $\q_1, \dots, \q_t$. Then $\g \perp \spanof\{\q_1, \dots, \q_t\}$.
\label{th:g_orth}
\end{lemma}
% \begin{proof}
%     After the weight correction step $\weights$ is a stationary point of $R(\Q(\cdot))$, i.e., we have for all $j \in [t]$
%     \begin{equation*}
%         0 = \frac{\partial R(\Q\weights)}{\partial \beta_j}
%           = \sum_{i=1}^n \frac{\partial\, l(\inner{\tilde{\q}_i}{\weights}, y_i)}{\partial \beta_j} 
%           = \sum_{i=1}^n q_{ij} \underbrace{\frac{\partial\, l(\inner{\tilde{\q}_i}{\weights}, y_i)}{\partial\, \inner{\tilde{\q}_i}{\weights}}}_{g_i} = \inner{\q_j}{\g} \enspace .
%     \end{equation*}
% \end{proof}
Moreover, the right hand side of Eq.~\eqref{eq:gen_proj_error} is technically undefined for redundant query vectors $\q$ that lie in $\range\, \Q$ and therefore have $\|\q_\perp\|=0$.
Through Lm.~\ref{th:g_orth} we know that for such queries we also have $\inner{\g}{\q}=0$, which suggests to simply fix this issue by defining the objective value in this case to be $0$.
However, this solution would not fix numerical instabilities when $\|\q_\perp\|$ is close to zero.
A better solution is therefore to add a small positive value $\epsilon$ to the denominator, which can be considered a \defemph{regularization parameter}.
With this we arrive at the final form of our objective function, which we state along with some of its basic properties in the following theorem.
% (proof in SI~\citep{github_url}).
\begin{theorem}
Let $\Q = [\q_1, \dots, \q_{t-1}] \in \R^{n \times (t-1)}$ be the selected query matrix and $\g$ the corresponding gradient vector after full weight correction, and let us denote by $\q=\q_\perp+\q_\parallel$ the orthogonal decomposition of $\q$ with respect to $\range\, \Q$. 
%, and $\q^*$ a maximizer of the \defemph{orthogonal gradient boosting objective} 
% $
%     \ogbobj(q) = |\inner{\g}{\q}|/(\|\q_\perp\|+\epsilon)
% $
% where $\q_\perp$ is the projection of $\q$ onto the orthogonal complement of $\range \,\Q$. 
Then we have for a maximizer $\q^*$ of the \defemph{orthogonal gradient boosting objective} 
$
    \ogbobj(q) = |\inner{\g}{\q}|/(\|\q_\perp\|+\epsilon)
$:
\begin{itemize}
    \item[a)] For $\epsilon \to 0$, $\spanof\{\q_1, \dots, \q_{t-1}, \q^*\}$ is the best approximation to $\spanof\{\q_1, \dots, \q_{t-1}, \g\}$.
    % as defined in~\eqref{eq:gen_proj_error}.
    % \item[b)] For $\epsilon \to \infty$, $\q^*$ is a maximizer of $\gsobj$ and any maximizer of $\gsobj$ is a maximizer of $\ogbobj$.
    \item[b)] For $\epsilon \to \infty$, $\q^*$ maximizes $\gsobj$ and any maximizer of $\gsobj$ maximizes $\ogbobj$.
    \item[c)] For $\epsilon = 0$ and $\|\q_\perp\|>0$, the ratio $(\ogbobj(q)/\gbobj(q))^2$ is equal to $1+(\|\q_\parallel\|/\|\q_\perp\|)^2$.
    \item[d)] The objective value $\ogbobj(q)$ is upper bounded by $\|\g\|$.
\end{itemize}
    \label{thm:objective}
\end{theorem}
% \begin{comment}
% \begin{proof}
% %Pierre's attempt at proving b).
% Suppose that for $\epsilon \geq 0$, $q^* \in \argmax_q \ogbobj(q)$, and for any $q' \in \argmax_q \gsobj(q)$, we have $\frac{\gsobj(q')}{\|\q'_\perp\|+\epsilon} < \frac{\gsobj(q^*)}{\|\q^*_\perp\|+\epsilon}$.
% Then $\frac{\gsobj(q')}{\|\q'_\perp\|+\epsilon'} \geq \frac{\gsobj(q^*)}{\|\q^*_\perp\|+\epsilon'}$ if and only if $\epsilon' \geq \frac{\|\q'_\perp\|\gsobj(q^*) - \gsobj(q')\|\q^*_\perp\|}{\gsobj(q') - \gsobj(q^*)}$.
% Therefore, if $q^*$ is a maximizer of $\ogbobj$ for $\epsilon$, but not of $\gsobj$, there exists an $\epsilon'$ such that $q^*$ is not a maximizer of $\ogbobj$. We conclude that for large enough $\epsilon$, only maximizers of $\gsobj$ can be maximizers of $\ogbobj$.
% \end{proof}
% \end{comment}

% If there is a fully weight-correction step in each iteration of boosting, the weights of all rules are changed. However, the selected queries may not be the best after the weight-correction if the weight correction step is not considered during selection of queries. 

% Figure \ref{fig:subspace} shows two approximations to the subspace spanned by the existing query $\textbf{q}_1$ and the negative gradient vector $-\textbf{g}$. $\textbf{q}_2$ is more closed to $-\textbf{g}$ than $\textbf{q}_3$, and therefore it is preferred by the objective function \eqref{eq:gb_obj} of gradient boosting. However, the subspace $\text{span}\{\textbf{q}_1, \textbf{q}_3\}$ is more closed to $\text{span}\{\textbf{q}_1, \textbf{g}\}$ than $\text{span}\{\textbf{q}_1, \textbf{q}_2\}$.

% \begin{proposition} \label{th:gb_not_best}
% In the subspace of complete ensemble coefficients, the objective function of gradient boosting \eqref{eq:gb_obj} does NOT identify the best geometric approximation to the subspace spanned by existing queries and the gradient.
% \end{proposition}

% Proposition \ref{th:gb_not_best} indicates that we have to take into consideration the weight-correction step. Therefore, it requires a new objective function to select the most suitable queries.
% In this section, we introduce the novel objective function which is used in our approach.

% Figure \ref{fig:orth_demo} demonstrates the idea of the orthogonal projection in the proposed algorithm. 
% There are three data points in the 3-D space, and a rule $w_1q_1$ covering both $(x_1, y_1) $ and $(x_2, y_2)$ is learned already.  
% If there are two candidate queries, $q_2$ and $q_3$, as shown in the figure, and $q_2$ covers only one data point $(x_3, y_3)$, while $q_3$ covers both $(x_1, y_1)$ and $(x_3, y_3)$.
% Before the orthogonal projection, the query $q_2$ is more closed to the negative gradient vector $-\textbf{g}$ than $q_3$.
% However, if we have a fully-corrective step, actually the component of the candidate queries parallel to the subspace spanned by the existing rules does not affect the prediction. 
% Therefore, we can calculate the component of the queries which affect the output of the model by calculating the orthogonal projection of the queries. 
% (Here``orthogonal projection'' means the projection of the query onto the subspace orthogonal to all the existing rules.)
% We can see that the orthogonal projection of $q_2'$ is closer to the negative gradient vector $-\textbf{g}$ than the orthogonal projection of $q_2$. 


% If there are already $k$ rules learned, we define the query matrix across all the data points as \eqref{eq:query_matrix}:
% \begin{equation}\label{eq:query_matrix}
%     Q_k=\left[\textbf{q}_1,..., \textbf{q}_k\right], 
% \end{equation}
% where $\textbf{q}_i = [q_i(x_1), ... q_i(x_n)]^T$ is the output vector of the $i$th query.



% The projection of a query $\textbf{q}$ on the subspace orthogonal to the existing queries is calculated by \eqref{eq:orth_proj}:
% \begin{equation}\label{eq:orth_proj}
%     \textbf{q}_\bot=\left(I-Q_k(Q_k^TQ_k)^{-1}Q_k^T\right)\textbf{q}.
% \end{equation}
% The objective function is
% \begin{equation}\label{eq:orth_obj}
%     \text{obj}_{\text{orth}}(\textbf{q})=\frac{|\textbf{q}_\bot\cdot\textbf{g}|}{\norm{\textbf{q}_\bot}},
% \end{equation}
% where $$\textbf{g}=\left[\frac{\partial l(f(x_1), y_1)}{\partial f(x_1)}, \dots, \frac{\partial l(f(x_n), y_n)}{\partial f(x_n)}\right]^T.$$

Intuitively, the orthogonal gradient boosting objective function measures the cosine of the angle between the gradient vector and the orthogonal projection of a candidate query vector $\q$. This is in contrast to the standard gradient boosting objective, which considers the angle of the unprojected query vector instead. 
In the example in Fig.~\ref{fig:subspace} we can observe that this difference leads to successfully identifying the best approximating subspace, and
Thm.~\ref{thm:objective}a) guarantees this property.

\begin{algorithm}[tb]
   \caption{FCOGB}%{Fully-corrective Orthogonal Gradient Boosting}
   \label{alg:fcogb}
\begin{algorithmic}
   \STATE {\bfseries Input:} dataset $(x_i, y_i)_{i=1}^{n}$, number of rules $k$
   \STATE Initialise $f^{(0)}=0$
   \FOR{$t=1$ {\bfseries to} $k$}
   \STATE $\textbf{g}=\left(\frac{\partial l(f^{(t-1)}(x_1), y_1)}{\partial f^{(t-1)}(x_1)}, \dots, \frac{\partial l(f^{(t-1)}(x_n), y_n)}{\partial f^{(t-1)}(x_n)}\right)$
   \STATE $q_t=\argmax_{q \in \cQ}{\frac{|\inner{\q}{\g}|}{\|\q_\perp\|}}$ \hfill//beam or bb search% \texttt{beam}($\g$, $\matO_{t-1}$) or \texttt{bb}($\g$, $\matO_{t-1}$)
   \STATE $\veco_t=\q_{t\perp}/\|\q_{t\perp}\|$ and $\matO_{t}=[\matO_{t-1}; \veco_t]$
   \STATE $\weights_t = \argmin_{\weights \in \R^t}{R([\q_1, \dots, \q_t]\weights)}$ \hfill//convex opt% via \texttt{convex\_opt}
   \STATE $f^{(t)}=[\q_1, \dots, \q_t]\weights_t$ %\left\{\textbf{q}^{(1)}_*, \dots, \textbf{q}^{(t)}_*\right\}\textbf{w}^{(t)}_*$
   \ENDFOR
   \STATE {\bfseries Output:} $f^{(k)}(\cdot)=\beta_{k, 1}q_1(\cdot)+\dots+\beta_{k, k}q_k(\cdot)$
\end{algorithmic}
\end{algorithm}

% Now we show that the objective function of the proposed algorithm identifies the subspace spanned by existing queries and the new query approximates best geometrically to the subspace spanned by existing queries and the gradient.
% \begin{theorem}
% The orthogonal objective function~\eqref{eq:orth_obj} identifies a vector $\hat{\textbf{q}}$ such that 
% for any vector $\textbf{v}^{(g)}\in\text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k, \textbf{g}\}$
% there exists a vector $\hat{\textbf{v}}\in\text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k, \hat{\textbf{q}}\}$ which satisfies
% \begin{equation*}
%     \norm{\textbf{v}^{(g)}-\hat{\textbf{v}}}=\min_{\textbf{q}}\left(\min_{\textbf{v}\in\text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k, \textbf{q}\}}\norm{\textbf{v}^{(g)}-\textbf{v}}\right).
% \end{equation*}
% \end{theorem}
% \begin{proof}
% For any vector \textbf{g} and $\textbf{q}$, they can be written as 
% $\textbf{g}=\textbf{g}_Q+\textbf{g}_\bot$
% and $\textbf{q}=\textbf{q}_Q+\textbf{q}_\bot, $ where $\textbf{g}_Q,\textbf{q}_Q \in \text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k\}, $
% and both $\textbf{g}_\bot$ and $\textbf{q}_\bot$ are in the subspace orthogonal to $\text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k\}$.

% Let $\textbf{v}^{(g)}=[Q^{(k)}; \textbf{g}]\textbf{w}^{(g)}$
% and $\textbf{v}^{(q)}=[Q^{(k)}; \textbf{q}]\textbf{w}^{(q)},$
% then
% \begin{align*}
%     &\norm{\textbf{v}^{(q)}-\textbf{v}^{(g)}}^2_2\\
%     =&\norm{[Q^{(k)}; \textbf{q}]\textbf{w}^{(q)}-[Q^{(k)}; \textbf{g}]\textbf{w}^{(g)}}_2^2\\
%     =&\norm{[Q^{(k)}; \textbf{q}_Q]\textbf{w}^{(q)}+w_{k+1}^{(q)}\textbf{q}_\perp-[Q^{(k)};\textbf{g}_Q] \textbf{w}^{(g)}-w_{k+1}^{(g)}\textbf{g}_\perp}_2^2\\
%     =&\norm{[Q^{(k)}; \textbf{q}_Q]\textbf{w}^{(q)}-[Q^{(k)};\textbf{g}_Q] \textbf{w}^{(g)}}_2^2+\\
%     &\norm{w_{k+1}^{(q)}\textbf{q}_\perp-w_{k+1}^{(g)}\textbf{g}_\perp}_2^2\\
% \end{align*}

% Since $\textbf{g}_Q,\textbf{q}_Q \in \text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k\},$ 
% these two vectors can be the same.
% Therefore, 
% \begin{align}\label{eq:min_diff_norm}
%     &\min\norm{\textbf{v}^{(q)}-\textbf{v}^{(g)}}_2^2\\
%     =&\min\norm{w_{k+1}^{(q)}\textbf{q}_\perp-w_{k+1}^{(g)}\textbf{g}_\bot}_2^2\\
%     \intertext{setting $\alpha=w_{k+1}^{(q)}/w_{k+1}^{(g)}$and $\gamma = w_{k+1}^{(g)}$}
%     =&\min\norm{\alpha\textbf{q}_\perp - \textbf{g}_\bot}_2^2 \gamma^2\\
%     =&\min\left(\textbf{g}_\bot\cdot\textbf{g}_\bot - 2\alpha\textbf{q}_{\perp}\cdot\textbf{g}_\bot+\alpha^2\textbf{q}_{\perp}\cdot\textbf{q}_\perp\right)\gamma^2 \\
%     \intertext{which is minimized for $\alpha=\textbf{q}_{\perp}\cdot\textbf{g}_\bot/\textbf{q}_{\perp}\cdot\textbf{q}_{\perp} $}=&\min\left(\textbf{g}_\bot\cdot\textbf{g}_\bot-\frac{\left(\textbf{q}_{\perp}\cdot\textbf{g}_\bot\right)^2}{\textbf{q}_{\perp}\cdot\textbf{q}_\perp}\right)\gamma^2,
% \end{align}
% Because of Lemma \ref{th:g_orth}, $\textbf{g}$ is always same as $\textbf{g}_\bot$.
% Therefore, maximising
% $
%     \cfrac{\left(\textbf{q}_{\perp}\cdot\textbf{g}\right)^2}{\norm{\textbf{q}_{\perp}}_2^2}
% $
% or 
% $
%     \cfrac{\left|\textbf{q}_{\perp}\cdot\textbf{g}\right|}{\norm{\textbf{q}_{\perp}}_2}
% $
% finds the vector $\hat{\textbf{q}}$ such that $\text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k, \hat{\textbf{q}}\}$
% best geometrically approximates
% $\text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k, \textbf{g}\}$.

% \end{proof}

% \input{4_1_table_updated.tex}
\subsection{Efficient Implementation}
%Having abstractly defined a rule objective function that is suitable in conjunction with full weight correction, we now turn to the question of how it can be computed efficiently in the context of the gradient boosting framework.
To develop an efficient optimization algorithm for the orthogonal gradient boosting objective, 
we recall that projections $\q_\perp$ on the orthogonal complement of $\range\,\Q$ can be naively computed via $\q_\perp=\Q((\Q^T\Q)^{-1}(\Q^T\q))$
% $
%     \q_\perp = \q - \underbrace{\Q((\Q^T\Q)^{-1}(\Q^T\q))}_{\q_\parallel}
% $
where we placed the parentheses to emphasize that only matrix-vector products are involved in the computation---at least once the inverse of the Gram matrix $\Q^T\Q$ is computed.
This approach allows to compute projections, and thus objective values, in time $O(nt+t^2)$ per candidate query after an initial preprocessing per boosting round of cost $O(t^2n + t^3)$.

%While the dependencies on $t$ might seem negligible 
In a first step, this naive approach can be improved by maintaining an orthonormal basis of the range of the query matrix throughout the boosting rounds, resulting in a Gram-Schmidt-type procedure. Since the projections $\q_{t \perp}$ of the selected queries naturally form an orthogonal basis of $\range\, \Q$ this only requires normalization, which can be done essentially without additional cost. Formally, by storing $\veco_t = \q_{t\perp} / \|\q_{t\perp}\|$ in all boosting rounds $t$, subsequent projections can be computed via
$
    \q_\perp = \q - \matO(\matO^T\q)
    % \label{eq:proj_with_O}
$
where $\matO=[\veco_1, \dots, \veco_t]$.
This reduces the computational complexity per candidate query to $O(tn)$ without  additional preprocessing.

While this looks like the optimal complexity for evaluating $\ogbobj$ in isolation, it leads to a prohibitive complexity for large $n$ for finding the optimal query in a given round.
Specifically, branch-and-bound with the tight bounding function~\eqref{eq:tight_bound} evaluates $O(n)$ queries per expanded search node  and beam search even $O(d^2n)$.
In both cases, using the expression for $\q_\perp$ above repeatedly results in a quadratic cost in $n$ per search node.
To avoid this, we can exploit the structure of candidate evaluations, similar to other efficient rule and tree learning algorithms~\citep{mampaey2015efficient}. 

The candidates evaluated per search node of both branch-and-bound and beam search have query vectors that are prefixes of an ordered sub-selection of data points, 
in beam search because optimum cut-off values are sought for each of the $d$ input variables,
in branch-and-bound because the optimum in Eq.~\eqref{eq:tight_bound} is attained or  approximated by a prefix with respect to some presorting order. 
% (e.g., based on $g_i$ for the gradient boosting objective or $g_i/h_i$ for the extreme gradient boosting objective.
Hence, we need to solve the following \defemph{prefix optimization problem}: given an ordered sub-selection of $l$ of the $n$ data points, represented by an injective map $\sigma\from \{1, \dots, l\} \to \{1, \dots, n\}$, find the optimal prefix 
\begin{equation}
 i_* = \argmax_{i \in \{1, \dots, l\}} \frac{\inner{\g}{\q^{(i)}}}{\|\q^{(i)}_\perp\| + \epsilon} 
 \label{eq:best_prefix}
\end{equation}
where $\q^{(0)}=\0$ and $\q^{(i)}=\q^{(i-1)}+\e_{\sigma(i)}$.
%A naive solution to this problem is to compute the projection matrix $\M=\I-\matO\matO^T \in \R^{n \times n}$ with $\matO=[\veco_1,\dots, \veco_t]$ and use it to compute the projection $\q^{(i)}_\perp = \M\q^{(i)}$ of all $i$ prefixes to find the maximum in Eq.~\eqref{eq:best_prefix}.
%While this approach is straightforward to implement, its computational complexity is of order $O(n^3)$, given that usually $l \approx n$, because it requires the computation of $l$ matrix-vector products involving an $n$-by-$n$ matrix. 
The following proof shows how the computational complexity for solving~\eqref{eq:best_prefix} can be substantially reduced compared to the direct approach above. 
It uses an incremental computation of projections that works directly on the available orthonormal basis vectors $\veco$ instead of computing matrix-vector products or, even worse, the whole projection matrix.
\begin{theorem}
    Given a gradient vector $\g \in \R^n$, an orthonormal basis $\veco_1, \dots, \veco_t \in \R^n$ of the subspace spanned by the queries of the first $t$ rules, and a sub-selection of $l$ candidate points $\sigma\from [l] \to [n]$, the best prefix selection problem~\eqref{eq:best_prefix} can be solved in time $O(tl)$.
    \label{thm:fast_prefix}
\end{theorem}
\begin{proof}[Proof sketch]
    We write the objective value of prefix $i$ in terms of incrementally computable quantities:
    \begin{align*}
        &\frac{\inner{\g}{\q^{(i)}}}{\|\q^{(i)}_\perp\| + \epsilon} = \frac{\inner{\g}{\q^{(i)}}}{\|\q^{(i)}\| - \|\q^{(i)}_\parallel\| + \epsilon} \\= &\frac{\inner{\g}{\q^{(i)}}}{\|\q^{(i)}\| - \sqrt{\sum_{k=1}^t \|\veco_k \veco_k^T\q^{(i)}\|^2} + \epsilon}
        \enspace .
    \end{align*}
    In particular, the $t$ sequences of norms $\|\veco_k \veco_k^T\q^{(i)}\|$ can be computed in time $O(l)$ via cumulative summation of the $k$-th basis vector elements in the given order:
    \begin{align*}
        \|\veco_k\veco_k^T\q^{(i)}\|
        %=\left\|\veco_k\veco_k^T\left(\sum_{j=1}^i\e_{\sigma(j)}\right)\right\|
        =\|\veco_k\| \sum_{j=1}^i \inner{\veco_k}{\e_{\sigma(j)}}
        =\sum_{j=1}^i o_{k, \sigma(j)} 
    \end{align*}
    %To incrementally compute $\|q^{(i)}\|$  in time $O(t)$ per $i \in [n]$ as required by the claim we reduce the problem
\end{proof}
% \begin{proof}
%     To see the claim, we first rewrite the objective value for the $i$-th prefix as
%     \begin{equation*}
%         \frac{\inner{\g}{\q^{(i)}}}{\|\q^{(i)}_\perp\| + \epsilon} = \frac{\inner{\g}{\q^{(i)}}}{\|\q^{(i)}\| - \|\q^{(i)}_\parallel\| + \epsilon} 
%         \enspace .
%     \end{equation*}
%     The value of $\|\q^{(i)}\|$ is trivially given as $\sqrt{i}$, and $\inner{\g}{\q^{i}}$ can be easily computed for all $i \in [l]$ in time $O(n)$ via cumulative summation.
%     Finally we can reduce the problem of computing the (squared) norms of the $l$ projected prefixes to computing the $t$ (squared) norms of the prefixes on the subspaces given by the individual orthonormal basis vectors via
%     \begin{equation*}
%         \|\q^{(i)}_\parallel\|^2 = \left\|\sum_{k=1}^t \veco_k \veco_k^T\q^{(i)}\right\|^2 = \sum_{k=1}^t \|\veco_k \veco_k^T\q^{(i)}\|^2 \enspace .
%     \end{equation*}
%     Each of these $t$ sequences of (squared) norms can be computed in time $O(n)$ by rewriting
%     \begin{align*}
%         \|\veco_k\veco_k^T\q^{(i)}\| &= \left\|\veco_k\veco_k^T\left(\sum_{j=1}^i\e_{\sigma(j)}\right)\right\|\\
%         &=\|\veco_k\| \sum_{j=1}^i \inner{\veco_k}{\e_{\sigma(j)}}\\
%         &=\sum_{j=1}^i o_{k, \sigma(j)} 
%     \end{align*}
%     where the last equality shows how an $O(n)$-computation is achieved via cumulative summation of the $k$-th basis vector elements in the order given by $\sigma$.
%     %To incrementally compute $\|q^{(i)}\|$  in time $O(t)$ per $i \in [n]$ as required by the claim we reduce the problem
% \end{proof}
We close this section with a pseudocode (Alg.~\ref{alg:fcogb}) that summarizes the main ideas of the orthogonal gradient boosting and refer to the literature for details about the beam-search/branch-and-bound step.

% To find the query which maximise the objective function, a branch-and-bound approach proposed by \citet{boley2021better} is adopted.
% According to Lemma \ref{th:g_orth}, $\inner{\g}{\q_Q}=0,$ so $\inner{\g}{\q_\bot}=\inner{\g}{\q}$. 
% Let $I(\q)$ represent the support set of $\q$, then

% If there is a fully weight-correction step in each iteration of boosting:

% \begin{align}
%     \text{bnd}(\textbf{q})=\max_{J\subseteq I(\q)}\frac{\max\sum_{i\in J}{g_i}}{\min\left\{\norm{\q'_\bot}_2:\norm{\q'}_1=|J|, I(\q')\subseteq I(\q)\right\}}.
% \end{align}

% \subsection{Orthogonal projection approach covers more data points}
% Theorem \ref{th:more_parallel} shows that with the orthogonal projection approach, the selected queries tend to select more data points covered by previous rules than the approach without orthogonal projection.
% \begin{lemma}\label{th:more_parallel}
% If
% \begin{equation}\label{eq:orth_obj_max}
%     \textbf{u}=\arg\max_{\textbf{q}}\frac{|\textbf{q}_\perp\cdot\textbf{g}|}{||\textbf{q}_\perp||}, 
% \end{equation}
% and 
% \begin{equation}\label{eq:gpe_obj_max}
%     \textbf{v}=\arg\max_{\textbf{q}}\frac{|\textbf{q}\cdot\textbf{g}|}{||\textbf{q}||},
% \end{equation}
% then
% \begin{equation}
%     \frac{||\textbf{v}_\perp||}{||\textbf{v}_{\mathbin{\!/\mkern-5mu/\!}} ||}\geq\frac{||\textbf{u}_\perp||}{||\textbf{u}_{\mathbin{\!/\mkern-5mu/\!}} ||}.
% \end{equation}
% \end{lemma}
% \begin{proof}

% From \eqref{eq:orth_obj_max}, we get
% \begin{equation}
% \frac{\left|\textbf{u}_\perp\cdot\textbf{g}\right|}{||\textbf{u}_\perp||}\geq\frac{\left|\textbf{v}_\perp\cdot\textbf{g}\right|}{||\textbf{v}_\perp||},
% \end{equation}
% which means 
% \begin{equation}
%     \frac{\left|\textbf{u}_\perp\cdot\textbf{g}\right|}{\left|\textbf{v}_\perp\cdot\textbf{g}\right|}\geq\frac{||\textbf{u}_\perp||}{||\textbf{v}_\perp||}.
% \end{equation}
% From \eqref{eq:gpe_obj_max}, we get
% \begin{equation}
% \frac{\left|\textbf{v}\cdot\textbf{g}\right|}{\sqrt{||\textbf{v}_\perp||^2+||\textbf{v}_{\mathbin{\!/\mkern-5mu/\!}}||^2}}=
%     \frac{\left|\textbf{v}\cdot\textbf{g}\right|}{||\textbf{v}||}\geq\frac{\left|\textbf{u}\cdot\textbf{g}\right|}{||\textbf{u}||}
%     =\frac{\left|\textbf{u}\cdot\textbf{g}\right|}{\sqrt{||\textbf{u}_\perp||^2+||\textbf{u}_{\mathbin{\!/\mkern-5mu/\!}}||^2}},
% \end{equation}
% which means
% \begin{equation}
%     \frac{\sqrt{||\textbf{u}_\perp||^2+||\textbf{u}_{\mathbin{\!/\mkern-5mu/\!}}||^2}}{\sqrt{||\textbf{v}_\perp||^2+||\textbf{v}_{\mathbin{\!/\mkern-5mu/\!}}||^2}}
%     \geq\frac{\left|\textbf{u}\cdot\textbf{g}\right|}{\left|\textbf{v}\cdot\textbf{g}\right|}
% \end{equation}
% From Lemma \ref{th:g_orth} and Lemma \ref{th:eq_span}, we know
% \begin{equation}
%     \textbf{u}_{\mathbin{\!/\mkern-5mu/\!}}\cdot\textbf{g}=\textbf{v}_{\mathbin{\!/\mkern-5mu/\!}}\cdot\textbf{g}=0.
% \end{equation}
% Therefore,
% \begin{equation}
%     \textbf{u}\cdot\textbf{g}=\textbf{u}_\perp\cdot\textbf{g}+\textbf{u}_{\mathbin{\!/\mkern-5mu/\!}}\cdot\textbf{g}=\textbf{u}_\perp\cdot\textbf{g}.
% \end{equation}

% In the end, we can conclude that
% \begin{equation*}
%     % ||\textbf{u}_{\mathbin{\!/\mkern-5mu/\!}}||\geq||\textbf{v}_{\mathbin{\!/\mkern-5mu/\!}} ||?
%     \frac{||\textbf{v}_\perp||}{||\textbf{v}_{\mathbin{\!/\mkern-5mu/\!}} ||}\geq\frac{||\textbf{u}_\perp||}{||\textbf{u}_{\mathbin{\!/\mkern-5mu/\!}} ||}
% \end{equation*}

% \end{proof}


==> 4_1_table_fix_obj.tex <==
\begin{table}
\caption{(Temp) Comparison of normalised risks and computation times for rule ensembles, averaged over cognitive complexities between 1 and 50, using SIRUS(SRS), Gradient Sum(GS), Gradient boosting (GB), XGBoost (XGB) and FCOGB (OB), for benchmark datasets of classification (upper), regression (middle) and Poisson regression problems (lower).}
\label{tb:comparison}
\vskip 0.05in
% \hskip 0.05in
\begin{center}
\begin{scriptsize}
\begin{sc}
\begin{tabular}{l@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c}
\toprule
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{8}{c}{Train risks} & \multicolumn{8}{c}{Test risks} \\
\multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & \multicolumn{1}{c}{\multirow{-2}{*}{$d$}} & \multicolumn{1}{c}{\multirow{-2}{*}{$n$}} & SRS & GS & GB & XGB & OB$_{Gr}$ & OB$_{BB}$ & OB$_{Fix}$ & \multicolumn{1}{l}{Improved} & SRS & GS & GB & XGB & OB$_{Gr}$ & OB$_{BB}$ & OB$_{Fix}$ & \multicolumn{1}{l}{Improved} \\
\midrule
titanic & 7 & 1043 & .895 & .653 & .656 & .646 & {\color[HTML]{FF0000} .639} & {\color[HTML]{FF0000} .621} & {\color[HTML]{FF0000} \textbf{.616}} & Y & .894 & .695 & .707 & .711 & .713 & {\color[HTML]{FF0000} \textbf{.695}} & .717 & N \\
tic-tac-toe & 27 & 958 & .892 & .555 & .641 & .577 & .650 & {\color[HTML]{FF0000} .506} & {\color[HTML]{FF0000} \textbf{.492}} & Y & .885 & .596 & .682 & .629 & .721 & {\color[HTML]{FF0000} .577} & {\color[HTML]{FF0000} \textbf{.566}} & Y \\
iris & 4 & 150 & .685 & .261 & .261 & .332 & {\color[HTML]{FF0000} \textbf{.192}} & {\color[HTML]{FF0000} .251} & {\color[HTML]{FF0000} .251} & Y & .745 & .521 & .440 & .459 & .531 & {\color[HTML]{FF0000} \textbf{.424}} & {\color[HTML]{FF0000} \textbf{.424}} & Y \\
breast & 30 & 569 & .569 & \textbf{.277} & .310 & .314 & .290 & .304 & .304 & Y & .627 & \textbf{.269} & .362 & .338 & .383 & .349 & .349 & Y \\
wine & 13 & 178 & .578 & .216 & .250 & .192 & {\color[HTML]{FF0000} .191} & {\color[HTML]{FF0000} .183} & {\color[HTML]{FF0000} \textbf{.183}} & Y & .621 & .346 & .431 & .409 & .483 & {\color[HTML]{FF0000} \textbf{.250}} & {\color[HTML]{FF0000} .265} & N \\
ibm hr & 32 & 1470 & .980 & .567 & .560 & .571 & {\color[HTML]{FF0000} .558} & {\color[HTML]{FF0000} \textbf{.553}} & {\color[HTML]{FF0000} .558} & N & .974 & .640 & .645 & .636 & .652 & {\color[HTML]{FF0000} \textbf{.617}} & {\color[HTML]{FF0000} .621} & N \\
telco churn & 18 & 7043 & .944 & .679 & .682 & .678 & {\color[HTML]{FF0000} \textbf{.664}} & {\color[HTML]{FF0000} .667} & {\color[HTML]{FF0000} .668} & N & .945 & .663 & .677 & .665 & {\color[HTML]{FF0000} \textbf{.650}} & {\color[HTML]{FF0000} .653} & {\color[HTML]{FF0000} .660} & N \\
gender & 20 & 3168 & .566 & .230 & .230 & .249 & {\color[HTML]{FF0000} .224} & {\color[HTML]{FF0000} .224} & {\color[HTML]{FF0000} \textbf{.224}} & Y & .570 & \textbf{.243} & .247 & .263 & .246 & .246 & .246 & Y \\
banknote & 4 & 1372 & .854 & .304 & .267 & .290 & {\color[HTML]{FF0000} .253} & {\color[HTML]{FF0000} .228} & {\color[HTML]{FF0000} .228} & Y & .858 & .311 & .268 & .299 & {\color[HTML]{FF0000} .264} & {\color[HTML]{FF0000} \textbf{.229}} & {\color[HTML]{FF0000} .229} & Y \\
liver & 6 & 345 & .908 & .815 & .834 & .814 & {\color[HTML]{FF0000} \textbf{.802}} & .854 & .834 & Y & .917 & .879 & .927 & \textbf{.873} & .940 & .924 & .891 & Y \\
magic & 10 & 19020 & .906 & .718 & .708 & .710 & {\color[HTML]{FF0000} .707} & {\color[HTML]{FF0000} .707} & {\color[HTML]{FF0000} .707} & Y & .903 & .698 & .693 & .693 & {\color[HTML]{FF0000} .688} & {\color[HTML]{FF0000} \textbf{.687}} & {\color[HTML]{FF0000} \textbf{.688}} & N \\
adult & 11 & 30162 & .804 & .594 & .599 & .588 & {\color[HTML]{FF0000} \textbf{.575}} & {\color[HTML]{FF0000} .576} & {\color[HTML]{FF0000} .576} & Y & .802 & .603 & .615 & .601 & {\color[HTML]{FF0000} \textbf{.589}} & {\color[HTML]{FF0000} .590} & {\color[HTML]{FF0000} .589} & Y \\
digits5 & 64 & 3915 & \textbf{.248} & .332 & .312 & .344 & .329 & .315 & .315 & Y & \textbf{.262} & .329 & .314 & .341 & .320 & .317 & .315 & Y \\
\midrule
insurance & 6 & 1338 & .169 & .130 & .142 & .144 & {\color[HTML]{FF0000} \textbf{.120}} & {\color[HTML]{FF0000} .127} & {\color[HTML]{FF0000} .123} & Y & .177 & .132 & .145 & .147 & {\color[HTML]{FF0000} \textbf{.127}} & {\color[HTML]{FF0000} .131} & {\color[HTML]{FF0000} .128} & Y \\
friedman1 & 10 & 2000 & .180 & .089 & .074 & .068 & {\color[HTML]{FF0000} .067} & {\color[HTML]{FF0000} \textbf{.065}} & {\color[HTML]{FF0000} .068} & N & .165 & .091 & .077 & .075 & {\color[HTML]{FF0000} \textbf{.070}} & {\color[HTML]{FF0000} .072} & {\color[HTML]{FF0000} .072} & Y \\
friedman2 & 4 & 10000 & .082 & .133 & .119 & .115 & {\color[HTML]{FF0000} .770} & .099 & {\color[HTML]{FF0000} \textbf{.075}} & Y & .082 & .135 & .120 & .115 & {\color[HTML]{FF0000} \textbf{.077}} & .102 & {\color[HTML]{FF0000} \textbf{.077}} & Y \\
friedman3 & 4 & 5000 & .093 & .045 & .042 & .042 & {\color[HTML]{FF0000} .041} & {\color[HTML]{FF0000} .041} & {\color[HTML]{FF0000} \textbf{.041}} & Y & .092 & .048 & .047 & .046 & {\color[HTML]{FF0000} .045} & {\color[HTML]{FF0000} .045} & {\color[HTML]{FF0000} \textbf{.045}} & Y \\
wage & 5 & 1379 & .427 & .370 & .362 & .359 & {\color[HTML]{FF0000} .352} & {\color[HTML]{FF0000} \textbf{.348}} & {\color[HTML]{FF0000} .354} & N & \textbf{.341} & .358 & .405 & .411 & .368 & .365 & .365 & Y \\
demographics & 13 & 6876 & .219 & .214 & .214 & .214 & {\color[HTML]{FF0000} .212} & {\color[HTML]{FF0000} \textbf{.212}} & {\color[HTML]{FF0000} \textbf{.212}} & Y & \textbf{.209} & .216 & .217 & .217 & .214 & .215 & .215 & Y \\
gdp & 1 & 35 & .063 & .020 & .020 & .020 & .024 & {\color[HTML]{FF0000} \textbf{.020}} & {\color[HTML]{FF0000} \textbf{.020}} & Y & .059 & .020 & .020 & .020 & .027 & {\color[HTML]{FF0000} \textbf{.020}} & {\color[HTML]{FF0000} \textbf{.020}} & Y \\
used cars & 4 & 1770 & .373 & .139 & .123 & .132 & {\color[HTML]{FF0000} \textbf{.113}} & .132 & {\color[HTML]{FF0000} \textbf{.121}} & Y & .427 & .171 & .131 & .141 & {\color[HTML]{FF0000} \textbf{.116}} & {\color[HTML]{FF0000} .130} & {\color[HTML]{FF0000} .130} & Y \\
diabetes & 10 & 442 & .156 & .138 & .142 & .139 & {\color[HTML]{FF0000} .132} & {\color[HTML]{FF0000} \textbf{.132}} & {\color[HTML]{FF0000} .134} & N & .188 & .141 & .141 & .147 & {\color[HTML]{FF0000} \textbf{.136}} & .148 & .149 & N \\
boston & 13 & 506 & .101 & .086 & .087 & .086 & {\color[HTML]{FF0000} \textbf{.080}} & {\color[HTML]{FF0000} .081} & {\color[HTML]{FF0000} .082} & N & .105 & \textbf{.079} & .087 & .089 & .088 & .087 & .087 & Y \\
happiness & 8 & 315 & .109 & .031 & .031 & .031 & {\color[HTML]{FF0000} .029} & {\color[HTML]{FF0000} \textbf{.029}} & {\color[HTML]{FF0000} \textbf{.029}} & Y & .109 & .033 & .039 & .039 & .035 & {\color[HTML]{FF0000} \textbf{.033}} & {\color[HTML]{FF0000} \textbf{.033}} & Y \\
life expect. & 21 & 1649 & .109 & .026 & .026 & .026 & {\color[HTML]{FF0000} .026} & {\color[HTML]{FF0000} .026} & {\color[HTML]{FF0000} .026} & Y & .110 & .027 & .027 & .027 & {\color[HTML]{FF0000} .026} & {\color[HTML]{FF0000} \textbf{.026}} & {\color[HTML]{FF0000} \textbf{.026}} & Y \\
mobile prices & 20 & 2000 & .148 & .131 & .137 & .137 & {\color[HTML]{FF0000} \textbf{.122}} & .134 & {\color[HTML]{FF0000} .126} & Y & .140 & .134 & .143 & .143 & {\color[HTML]{FF0000} \textbf{.126}} & .139 & {\color[HTML]{FF0000} .132} & Y \\
suicide rate & 5 & 27820 & .547 & .543 & .540 & .540 & {\color[HTML]{FF0000} .540} & {\color[HTML]{FF0000} \textbf{.531}} & {\color[HTML]{FF0000} .532} & N & .514 & .521 & .521 & .521 & {\color[HTML]{FF0000} .519} & {\color[HTML]{FF0000} \textbf{.509}} & {\color[HTML]{FF0000} .512} & N \\
videogame & 6 & 16327 & \textbf{.895} & .953 & .953 & .953 & .953 & .953 & .953 & Y & .850 & \textbf{.720} & \textbf{.720} & \textbf{.720} & {\color[HTML]{FF0000} \textbf{.720}} & {\color[HTML]{FF0000} \textbf{.720}} & {\color[HTML]{FF0000} \textbf{.720}} & Y \\
red wine & 11 & 1599 & .072 & .034 & .035 & .034 & {\color[HTML]{FF0000} .034} & {\color[HTML]{FF0000} .034} & {\color[HTML]{FF0000} .034} & Y & .073 & .035 & .036 & .036 & {\color[HTML]{FF0000} .035} & {\color[HTML]{FF0000} \textbf{.035}} & {\color[HTML]{FF0000} \textbf{.035}} & Y \\
\midrule
covid vic & 4 & 85 & NA & .153 & .121 & .132 & {\color[HTML]{FF0000} .105} & {\color[HTML]{FF0000} .105} & {\color[HTML]{FF0000} \textbf{.086}} & Y & NA & .182 & \textbf{.100} & .133 & .104 & .104 & .086 & Y \\
covid & 2 & 225 & NA & .344 & .371 & .891 & {\color[HTML]{FF0000} .343} & {\color[HTML]{FF0000} .335} & {\color[HTML]{FF0000} \textbf{.321}} & Y & NA & .459 & .411 & .741 & .417 & {\color[HTML]{FF0000} .407} & {\color[HTML]{FF0000} \textbf{.395}} & Y \\
bicycle & 4 & 122 & NA & .317 & .324 & .337 & {\color[HTML]{FF0000} .296} & {\color[HTML]{FF0000} .295} & {\color[HTML]{FF0000} \textbf{.275}} & Y & NA & .366 & .478 & .457 & .529 & {\color[HTML]{FF0000} .328} & {\color[HTML]{FF0000} \textbf{.320}} & Y \\
ships & 4 & 34 & NA & .174 & .181 & .146 & {\color[HTML]{FF0000} \textbf{.125}} & .186 & .168 & Y & NA & .197 & .203 & .199 & .464 & {\color[HTML]{FF0000} .172} & {\color[HTML]{FF0000} \textbf{.155}} & Y \\
smoking & 2 & 36 & NA & .127 & .128 & .163 & {\color[HTML]{FF0000} \textbf{.078}} & {\color[HTML]{FF0000} .091} & {\color[HTML]{FF0000} .072} & Y & NA & .136 & .250 & .322 & {\color[HTML]{FF0000} .121} & {\color[HTML]{FF0000} .103} & {\color[HTML]{FF0000} \textbf{.084}} & Y

\\

\bottomrule
\end{tabular}
\end{sc}
\end{scriptsize}
\end{center}
\vskip -0.2in
\end{table}


==> old/2_preliminaries.tex <==
\begin{figure*}[t!]
% \vskip 0.1in
\centering
\includegraphics[width=0.45\columnwidth]{Images/Subspaces.png}
\hspace{1cm}
\includegraphics[width=0.45\columnwidth]{Images/orth_demo.png} 
% \vskip -0.1in
\caption{
Illustration of output space for toy regression example with three data points with target values $y_1=-10$, $y_2=-6$, $y_3=5$ and three queries with output vectors $\q_1=(1, 1, 0)$, i.e., $q_1$ selects the first two data points, $\q_2=(0, 0, 1)$, and $\q_3=(0, 1, 1)$. The gradient boosting objective selects $q_1$ with weight $\beta_1=-8$ as first rule, resulting in a negative gradient vector $-\g=(-2, 2, 5)$.
\emph{Left:} Approximations~\eqref{eq:gen_proj_error} to target subspace (blue) spanned by $\q_1$ and $-\g$. The subspace (green) spanned by $\q_3$ and $\q_1$ is a better approximation than the subspace (orange) spanned by $\q_2$ and $\q_1$.
However, the latter is selected by standard gradient boosting. %~\eqref{eq:gb_obj}.
\emph{Right:} After projection onto orthogonal complement of already selected query, angle between $\q_3$ and $-\g$ is smaller than that between $\q_2$ and $-\g$ and is thus successfully selected by orthogonal gradient boosting objective.}
\label{fig:subspace}
\end{figure*}
\section{Rule Boosting}\label{grb}

%\subsection{Rule ensembles, risk, and comprehensibility}
An \defemph{additive ensemble} of $k$ rules can be represented by Boolean query functions $q_1, \dots, q_k$ and a \defemph{weight vector} $\weights=(\weight_1, \dots, \weight_k)^T \in \R^k$
that jointly describe a function 
$
    f(\x) = \sum_{i=1}^{k}{\weight_i q_i(\x)}
$,
the output of which can be mapped to the conditional distribution of a target variable $Y | X=\x$.
That is, the queries define the rule antecedents (rule bodies), and the coefficients $\weights$ define the rule consequents, i.e., the output of rule $i$ for input $\x\in \R^d$ is $\weight_i$ if $\x$ satisfies the antecedent, i.e., $q_i(\x)=1$ (and $0$ otherwise).
Moreover, each \defemph{query function} $q_i\from \R^d \to \{0, 1\}$ is a conjunction of $c_i$  \defemph{propositions}, i.e., $q_i(\x)=p_{i,1}(\x)p_{i,2}(\x)\dots p_{i,c_i}(\x)$ where the $p_{i,j}$ are typically a threshold function on an individual input variable, e.g., $p_{i,j}(\x)=\delta(x_l \geq t)$.
We denote the set of available propositions by $\cP$ and the \defemph{query language} of all conjunctions that can be formed from $\cP$ as $\cQ$.
% \begin{equation*}
%     q_i = \bigwedge_{j=1}^{m_i}{p_j}, 
% \end{equation*}


We are concerned with two properties of an additive rule ensemble: its (empirical) prediction \defemph{risk}\footnote{Note that for all algorithms discussed here, the $l_2$-regularized risk can also be  considered with only light modifications. However, for ease of exposition, and since regularization typically is not crucial for the rather small rule ensembles considered here, we focus on the unregularized case.}
$
    R(f) = \frac{1}{n}\sum_{i=1}^{n}{l(f(\x_i), y_i)}
$,
measured by some positive loss function $l(f(\x), y)$ averaged over a dataset $\{(\x_1, y_1),\dots, (\x_n, y_n)\}$,
and its \defemph{cognitive complexity} $C(f) = k + \sum_{i=1}^k c_i$, measuring the cognitive effort required to parse all rule consequents and antecedents.
Here we consider loss functions that can be derived as negative log likelihood (or rather deviance function) when interpreting the rule ensemble output as natural parameter of an exponential family model of the target variable, which  guarantees that the loss function is strictly convex and twice differentiable.
%This has several advantages. Firstly, the resulting rule ensembles can be interpreted as probabilistic models that encode a conditional distribution $Y | X=x$. Hence, besides enabling predictions via $E[Y| X=x]$, they also provide calibrated uncertainty estimates.
%Moreover, it also guarantees that the loss function is strictly convex and twice differentiable. 
Specifically, we consider the cases of \defemph{squared loss} $l_\mathrm{sqr}(f(x_i), y_i) = (f(x_i)-y_i)^2$, the \defemph{logistic loss} $l_\mathrm{log}(f(x_i), y_i)=\log(1+\exp(-y_if(x_i)))$, and the \defemph{Poisson loss} $l_\mathrm{poi}(f(x_i), y_i)=y_i\log y_i-y_if(x_i)-y_i+\exp(f(x_i))$.
\begin{comment}
Specifically, we consider the cases of \defemph{squared loss} 
\begin{equation*}
l_\mathrm{sqr}(f(x_i), y_i) = (f(x_i)-y_i)^2
\end{equation*}
for regression problems where we model $Y | x$ as normally distributed with mean $f(x)$, \defemph{logistic loss} 
\begin{equation*}
l_\mathrm{log}(f(x_i), y_i)=\log(1+\exp(-y_if(x_i)))
\end{equation*}
for (binary) classification where we model $Y| x$ as Bernoulli distributed with positive probability $1/(1+\exp(-f(x)))$ and \defemph{Poisson loss} 
\begin{equation*}
l_\mathrm{poi}(f(x_i), y_i)=\log y_i-f(x_i)-y_i+\exp(f(x_i))
\end{equation*}
for count regression where we model $Y | x$ as Poisson distributed with mean $\exp(f(x))$.
\end{comment}

\paragraph{Gradient boosting}
Gradient boosting~\cite{friedman2001greedy} is a ``stagewise'' fitting scheme for additive models that, in our context, produces a sequence of rule ensembles $f^{(0)}, f^{(1)}, \dots, f^{(k)}$ such that $f^{(0)}(\x)= 0$ and, for $t \in [1, k]$, $f^{(t)}(\x)=f^{(t-1)}(\x)+\weight_t q_t(\x)$. 
%In other words, it is a greedy approach that fits one rule per iteration without correcting the previously fitted rules.
%Specifically, the seminal idea in \citet{friedman2001greedy} is to choose the query (or ``baselearner'') in iteration $t$ to perform an approximate gradient descent in $\R^n$---the model ``output space'' defined by the  training data. 
Specifically, the term $\weight_t q_t(\x)$ is chosen to perform an approximate gradient descent with respect to the risk function $R(f)=R(\f)$ considered as a function of the model \defemph{output vector} $\f=(f(\x_1),\dots, f(\x_n))$.
% This gradient $\g$ has components $g_i=\partial l(f(x_1), y_1) / \partial f(x_i)$
% a current model function $f$, we define the \defemph{gradient vector} as 
% \begin{equation}
%     \g = \left(\frac{\partial l(f(x_1), y_1)}{\partial f(x_1)}, \dots, \frac{\partial l(f(x_n), y_n)}{\partial f(x_n)}\right)^T
%     \label{eq:grad_vector}
% \end{equation}
% $\g=\nabla_{f(\textbf{x})}{R(f)}$
The exact gradient descent update would be $-\alpha_*\g$ where $\g$ is the \defemph{gradient vector} with components $g_i=\partial l(f(\x_i), y_i) / \partial f(\x_i)$ and $\alpha_*$ is the step length that minimizes the empicical risk $R(\f-\alpha\g)$.
%Here we consider $R(f)=R(\f)$ as a function of the model output and identify $f$ with its \defemph{output vector} $\f=(f(x_1),\dots, f(x_n))$.
However, since in general there is no query $q$ for which the output vector $\q=(q(x_1),\dots, q(x_n))$ is equal to the gradient $\g$, the goal is to select $\q^*$ that best approximates $\g$ in the sense that it minimizes the squared \defemph{projection error}
\begin{equation}
    \min_{\beta \in \R} \|-\!\alpha_* \g - \beta \q \|^2 = \alpha_*^2\left(\|\g\|^2 - \frac{(\inner{\q}{\g})^2}{\|\q\|^2}\right) \enspace .
    \label{eq:1d_proj_error}
\end{equation}
This is achieved by choosing $q_t$ to maximize the standard \defemph{gradient boosting objective}~\citep{dembczynski2010ender} $\gbobj(q)=|\inner{\q}{\g}| / \|\q\|$ and to find $\beta_{t} = \argmin_{\beta \in \R} R(\f + \beta\q_t)$ via a line search.
% Therefore, a direct implementation of gradient boosting for rule ensembles is achieved by the following updates that are used in~\citet{dembczynski2010ender}:
% \begin{align}
%     q_{t} = \argmax_{q \in \cQ} \underbrace{|\inner{\q}{\g}| / \|\q\|}_{\gbobj(q)}
%     \text{, }
%     \beta_{t} = \argmin_{\beta \in \R} R(\f + \beta\q_t) % \label{eq:gb_obj}
% \end{align}
% That is, the \defemph{gradient boosting objective} for query selection is to maximize the cosine (or minimize the angle) of the query output vector and the gradient vector.
Note that this $\beta_t$ is not generally equal to the minimizing $\beta$ in~\eqref{eq:1d_proj_error}, because the optimal update in direction $\q$ can be better than the best geometric approximation to the gradient descent update in direction $\q$.
A derivation of this objective function is the \defemph{gradient sum objective}~\citep{dembczynski2010ender, shalev2010trading} $\gsobj(q)=|\inner{\q}{\g}|$, 
which always selects more general rules than the gradient boosting objective~\citep[Thm.~1]{dembczynski2010ender}, however,  typically at the expense of an increased risk per rule, because the correction of data points with large gradient elements has to be toned down to avoid over-correction of other selected data points with small gradient elements.
Finally, an adaption of ``extreme gradient boosting''~\cite{chen2016xgboost} to rule ensembles yields the \defemph{extreme boosting objective}~\citep{boley2021better} $\xgbobj(q)=(\inner{\q}{\g})^2 / \inner{\q}{\h}$ 
where $\h=\text{diag}(\nabla^2_{f(\textbf{x})}{R(f)})$ is the diagonal vector of the risk Hessian  again with respect to the output vector $\f$.
This approach starts from the second order approximation of $R(\f + \beta\q)$ for which also yields a closed form weight update $\beta_{t} = -\inner{\q}{\g}/\inner{\q}{\h}$.
This approach is well-defined for our loss functions derived from exponential family response models, which guarantee defined and positive $\h$.
For the squared loss, it is equivalent to standard gradient boosting, because the second order approximation is exact for $l_\mathrm{sqr}$ and $\h$ is constant.
%A derivation of these updates discussed in both~\citet{dembczynski2010ender} and~\citet{shalev2010trading} is to drop the normalization $\|\q\|$ and instead use only the sum of selected gradient elements, i.e.,
% \begin{equation}
%     q_{t} = \argmax_{q \in \cQ} \underbrace{|\inner{\q}{\g}|}_{\gsobj(q)}\label{eq:gs_obj}
% \end{equation}
% which we refer to here as \defemph{gradient sum objective}.
% This variant always selects more general rules than the gradient boosting objective~\citep[Thm.~1]{dembczynski2010ender}, however,  typically at the expense of an increased risk per rule, because the correction of data points with large gradient elements has to be toned down to avoid over-correction of other selected data points with small gradient elements.

% A further variant of the original gradient boosting approach is ``extreme gradient boosting''~\cite{chen2016xgboost}, which is the basis of the additive rule ensemble algorithm presented in~\citet{boley2021better}. This approach starts from the second order approximation of $R(\f + \beta\q)$ for which the closed form solution yields the \defemph{extreme boosting objective} function and closed form weight updates
% \begin{align}
%     q_{t} = \argmax_{q \in \cQ} \underbrace{(\inner{\q}{\g})^2 / \inner{\q}{\h}}_{\xgbobj(q)}\text{, }
%     \beta_{t} = -\inner{\q}{\g}/\inner{\q}{\h} \label{eq:xgb_obj}
% \end{align}
% where $\h=\text{diag}(\nabla^2_{f(\textbf{x})}{R(f)})$ is the diagonal vector of the risk Hessian matrix again with respect to the output vector $\f$.
% \begin{equation*}
%     \h = \left(\frac{\partial^2 l(f(x_1), y_1)}{\partial f(x_1)^2}, \dots, \frac{\partial^2 l(f(x_1), y_1)}{\partial f(x_n)^2}\right)^T \enspace .
% \end{equation*}
%This approach is well-defined for our loss functions derived from exponential family response models, which, as mentioned above, guarantee that $\h$ is defined and has only positive components.
%Moreover, for the squared loss, the extreme boosting objective is equivalent to standard gradient boosting, because the second order approximation is exact for $l_\mathrm{sqr}$ and $\h$ is constant.
%the updates defined by~\eqref{eq:xgb_obj} are equivalent to those given by~\eqref{eq:gb_obj}

\paragraph{Single rule optimization}
%weight update can be done by Newton search
%remains: how to find query
%last decades ML literature: greedy optimization, designed for classification and regression trees for efficient generation of hundreds of trees (and thousands of rules)
%however, we are interested in small number of rules
%problem: misses the very interactions that are the reason why we prefer rule ensembles over simpler additive models like generalized linear models and generalized additive models
While the rule optimization literature can be neatly divided into heuristic (greedy / beam search) and exact branch-and-bound search, these approaches are actually closely related: they can both be described as traversing a lattice on the query language $\cQ$ imposed by a \defemph{specialization relation} $q \gen q'$ that holds if the propositions in $q'$ are a superset of those mentioned in $q$, and $q'$ thus logically implies $q$.
The difference between the approaches is under what conditions they discard specializations of candidate queries and how those specializations are generated.

Here, we build on the branch-and-bound framework presented in~\citet{boley2021better} that allows to efficiently search for optimal conjunctive queries in a condensed search space, given that there is an admissible, effective, and efficiently computable bounding function for the employed objective.
Specifically, let $\obj\from \cQ \to \R$ denote the objective function to be maximized. Then a \defemph{bounding function} $\bnd\from \cQ \to \R$ is  \defemph{admissible} if for all $q \in \cQ$ it holds that $\bnd(q) \geq \best(q)$ where 
% \begin{equation*}
$
    \best(q) = \max_{q \gen q' \in \cQ} \obj(q')
$
% \end{equation*}
denotes the objective value of the best specialization of $q$. A bounding function is effective in allowing to prune the search space if the difference $\bnd(q)-\best(q)$ tends to be small, rendering $\best(q)$ itself the theoretically most effective bounding function.
However, computing $\best(q)$ is as hard as the overall optimization problem.

A frequently applied recipe for constructing an admissible bounding function that is also effective and efficiently computable is to relax the quantifier in the definition of $\best$ and instead of bounding the value of the best specialization in the search space, bound the value of the best subset of data points of those selected by $q$~\citep{morishita2000transversing}. This results in the tight bounding function when \defemph{unaware of selectability}
\begin{equation}
\bnd(q) = \max\{\obj(\q'): \q' \leq \q, \q' \in \{0, 1\}^n\}\label{eq:tight_bound}
\geq \best(q) \enspace .
\end{equation}
Here, $\q \leq \q'$ refers to the component-wise less or equals relation on the binary output vector of $q$ and $q'$.
This function can be efficiently computed for many objective functions by pre-sorting the data in time $O(n \log n)$ that has to be carried out only once per fitted rule~\citep{lemmerich2016fast}. 
For instance for the extreme boosting objective, the optimum $q' \in \{0, 1\}^n$ can be found as a prefix or suffix of all data points after sorting them according to the ratio $g_i/h_i$ of first and second order loss derivatives.

%extreme ends: rulefit has very bad comprehensibility; other end recent approaches that fully optimize.
%inbetween: boosting-based approaches
%in this work we consesquently follow through with all choices required to fit rule ensembles for interpretability: full weight correction and optimal fitting

% \begin{equation*}
%     \f = [\q_1, \dots, \q_k]\weights
% \end{equation*}



%Old
%------------------
% \section{Gradient rule boosting}\label{grb}

% An additive rule ensemble can be represented as
% \begin{equation*}
%     f(x) = \sum_{i=1}^{k}{w_i q_i(x)}=\textbf{w}\cdot\textbf{q}(x),
% \end{equation*}
% where $q_i$ is a conjunction of $m_i$ boolean propositions:
% \begin{equation*}
%     q_i = \bigwedge_{j=1}^{m_i}{p_j}, 
% \end{equation*}
% and therefore, it is a boolean function as well.

% To learn an additive rule ensemble, given a set of training data $\{(x_i, y_i)\}_{i=1}^{n}$ which is drawn from the joint distribution of feature variables $X\in\mathbb{X}$ and output variable $Y\in\mathbb{Y}$, the goal is to find an additive rule ensemble with a number of components which minimises the risk function:
% \begin{equation*}
%     R(f) = \mathbb{E}_{X, Y}l(f(x_i), y_i),
% \end{equation*}
% where $l$ is a loss function. 
% The loss function measures the cost if the model output is $f(x)$ when the actual output is $y$, for example, squared loss $l(f(x_i), y_i) = (f(x_i)-y_i)^2$ is usually used for regression problems, logistic loss $l(f(x_i), y_i)=\log(1+\exp(-y_if(x_i)))$ is usually used for classification problems, and Poisson loss $l(f(x_i), y_i)=\log y_i-f(x_i)-y_i+\exp(f(x_i))$ is used for Poisson regression problems for counting outputs.

% However, usually the joint distribution of $X$ and $Y$ is unknown, so we use empirical risk instead:
% \begin{equation}
%     \hat{R}(f) = \frac{1}{n}\sum_{i=1}^{n}{l(f(x_i), y_i)}.
% \end{equation}

% Each iteration of boosting can be done in two steps: query selection and weight calculation. In the first step, a query is selected based on some objective functions. 
% After a query is chosen, we can calculate the weight of the query in a normal boosting framework, or we can also recalculate the weights of all existing queries in the rule ensemble.

% Gradient boosting is firstly introduced by \citet{friedman2001greedy}. 
% In each of its iterations, gradient boosting finds a query which satisfies:
% \begin{equation}\label{eq:gb_goal}
%     \min_\alpha {\norm{\alpha \textbf{q}^*-\textbf{g}}^2}=\min_{\alpha, \textbf{q}} {\norm{\alpha \textbf{q}-\textbf{g}}^2},
% \end{equation}
% where $\textbf{g}=\nabla \hat{R}(f)$ is the gradient vector of the current empirical risk in terms of the model's output. Equation \eqref{eq:gb_goal} yields the objective function of gradient boosting:
% \begin{equation}\label{eq:gb_obj}
%     \text{obj}_\text{gb}=\frac{|\textbf{q}\cdot\textbf{g}|}{\norm{\textbf{q}}},
% \end{equation}
% and this objective function should be maximised.

% If there is a vector $w^*_g\textbf{g}\in\text{span}\{\textbf{g}\}$, then \eqref{eq:gb_goal} finds the $\textbf{q}$ which minimises the distance between $w^*_g\textbf{g}$ and the subspace spanned by $\textbf{q}$. 
% Therefore, gradient boosting selects the base learner (query) which leads to the best geometric approximation of ensemble which adds $\textbf{g}$ with a risk-minimising weight.
% \begin{proposition}
% Gradient boosting identifies the 1d subspace spanned by a query $\textbf{q}$ which approximates best to the 1d subspace spanned by $\textbf{g}$.
% \end{proposition}

==> old/3_main_contributions.tex <==
\section{Fully-corrective Orthogonal Gradient Boosting}\label{fcogb}
% \begin{figure*}[t!]
% % \vskip 0.1in
% \centering
% \includegraphics[width=0.45\columnwidth]{Images/Subspaces.png}
% \hspace{1cm}
% \includegraphics[width=0.45\columnwidth]{Images/orth_demo.png} 
% % \vskip -0.1in
% \caption{
% Illustration of output space for toy regression example with three data points with target values $y_1=-10$, $y_2=-6$, $y_3=5$ and three queries with output vectors $\q_1=(1, 1, 0)$, i.e., $q_1$ selects the first two data points, $\q_2=(0, 0, 1)$, and $\q_3=(0, 1, 1)$. The gradient boosting objective selects $q_1$ with weight $\beta_1=-8$ as first rule, resulting in a negative gradient vector $-\g=(-2, 2, 5)$.
% \emph{Left:} Approximations~\eqref{eq:gen_proj_error} to target subspace (blue) spanned by $\q_1$ and $-\g$. The subspace (green) spanned by $\q_3$ and $\q_1$ is a better approximation than the subspace (orange) spanned by $\q_2$ and $\q_1$.
% However, the latter is selected by standard gradient boosting. %~\eqref{eq:gb_obj}.
% \emph{Right:} After projection onto orthogonal complement of already selected query, angle between $\q_3$ and $-\g$ is smaller than that between $\q_2$ and $-\g$ and is thus successfully selected by orthogonal gradient boosting objective.}
% \label{fig:subspace}
% \end{figure*}
%In this section, we firstly show the variant to boosting algorithm which recalculate all weights of existing rules in the generated ensemble, i.e. fully-corrective boosting. The objective function of gradient boosting cannot find the best approximation to the subspace spanned by existing queries and gradient in fully-corrective boosting. Therefore, we derive a novel objective function which takes the weight-correction step into consideration during the selection of queries. 

Having reviewed the existing rule boosting approaches, we now turn to improving them in terms of their risk/complexity trade-off.
Our approach to this is to improve the risk reduction per rule added to the ensemble, which directly affects the number of rules needed to achieve a certain risk. 
As it turns out, this typically coincides with preferring the addition of more general and hence simpler rules. 
Thus, it also positively affects the cognitive complexity on the level of the lengths of individual rules.

% \begin{figure}[tbh]
% \vskip 0.1in
% \centering
% \includegraphics[width=\columnwidth]{Images/orth_demo.png} 
% \caption{Illustration of orthogonal gradient boosting for a toy scenario with three data points (values marked with blue dots) corresponding to a three-dimensional output space: The negative risk gradient ($-g$, black) lies in the plane (highlighted in light blue) orthogonal to the already selected rule $w_1q_1$, which covers data points $x_1$ and $x_2$. For the second rule, the first candidate query ($q_2$, in orthogonal plane) covers only $x_3$ and is preferred by standard gradient boosting. The second candidate query ($q_3$) is more general, covering $x_2$ and $x_3$, but has a larger projection error initially. However, after orthogonalization ($q'_3$) it is preferred by orthogonal gradient boosting.}
% % output space for three datapoints 
% % already selected rule with query
% % gradient
% % two candidate queries for second rule
% % one (q1, already orthogonal to selected query) is closer to gradient and preferred by standard boosting
% % second (q2) is further away from gradient but closer after projection (dashed lione
% \label{fig:orth_demo}
% \vskip -0.1in
% \end{figure}

% \begin{figure*}[tbh]
% \vskip 0.1in
% \centering
% \includegraphics[width=\columnwidth]{Images/Subspaces.png}
% \includegraphics[width=\columnwidth]{Images/orth_demo.png} 
% \caption{
% Illustration of output space for toy regression example with three data points with target values $y_1=-10$, $y_2=-6$, $y_3=5$ and three queries with output vectors $\q_1=(1, 1, 0)$, i.e., $q_1$ selects the first two data points, $\q_2=(0, 0, 1)$, and $\q_3=(0, 1, 1)$. The gradient boosting objective selects $q_1$ with weight $\beta_1=-8$ as first rule, resulting in a negative gradient vector $-\g=(-2, 2, 5)$.
% \emph{Left:} Approximations~\eqref{eq:gen_proj_error} to target subspace (blue) spanned by $\q_1$ and $-\g$. The subspace (green) spanned by $\q_3$ and $\q_1$ is a better approximation than the subspace (orange) spanned by $\q_2$ and $\q_1$.
% However, the latter is selected by standard gradient boosting~\eqref{eq:gb_obj}.
% \emph{Right:} After projection onto orthogonal complement of already selected query, angle between $\q_3$ and $-\g$ is smaller than that between $\q_2$ and $-\g$ and is thus successfully selected by orthogonal gradient boosting objective.}
% \label{fig:subspace}
% \end{figure*}
\subsection{Weight Correction and Subspace Approximations}
A natural idea to reduce the ensemble risk per rule added is to relax the strict stagewise fitting approach of traditional gradient boosting and to allow the whole weight vector $\weights$ to be adjusted in every round $t$, i.e., to set
\begin{equation}
    \weights^{(t)} = \argmin_{\beta \in \R^t} R(\Q_t\weights) \enspace ,
    \label{eq:weight_correction}
\end{equation}
where $\Q_t=[\q_1, \dots, \q_t]$ is the $n\times t$ \defemph{query matrix} with the output vectors of all selected queries as columns.
In contrast to a full joint optimization of queries and weights, this intermediate solution still retains the computational benefits of gradient boosting for small rule ensembles:
Given that our loss function $l$ and therefore the empirical risk $R$ are convex, optimizing the weights in round $t$ is a convex optimization problem in $t$ variables, equivalent to fitting a small generalized linear model.
Using Newton-Raphson (``iterated least squares'') type algorithms, the computational cost of this is usually negligible compared to the more expensive query optimization step, especially when aiming for optimal individual queries for their reduced cognitive complexity.

Re-optimizing the weights, which is sometimes referred to as \defemph{fully corrective boosting}~\citep{shalev2010trading}, effectively turns boosting into a form of forward variable selection for linear models.
However, in contrast to conventional variable selection where all variables are given explicitly, we still have to identify a good query $q_t$ in each boosting iteration, 
and it turns out that finding the appropriate query is more complicated as in the case of single weight optimization characterized by~\eqref{eq:1d_proj_error}.
We still would like to add the direction of steepest descent, i.e., the negative gradient $-\g$, to the subsequent risk optimization step and approximate as closely as possible the outcome $[\Q_{t-1}; \g]\boldsymbol{\alpha}^*$ where $\alphavec^* \in \R^t$ are the risk minimizing weights for $\q_1, \dots, \q_{t-1}, \g$.
Therefore, the best approximating query $q$ is now given by
\begin{equation}
    \argmin_{q \in \cQ} \min_{\weights \in \R^t} \| [\Q_{t-1}; \g]\boldsymbol{\alpha}^* - [\Q_{t-1}; \q]\weights\|^2
    \label{eq:gen_proj_error} \enspace .
\end{equation}
It is an important observation that the standard gradient boosting objective does not correctly identify this optimally approximating query.
This is demonstrated by the example illustrated in Fig.~\ref{fig:subspace}.
In the left sub-figure it can be seen that the green plane, $\spanof\{\q_1, \q_3\}$, is a better approximation to $\spanof\{\q_1, -\g\}$ (blue) than the orange plain, $\spanof\{\q_1, \q_2\}$. However, the latter is selected by standard gradient boosting, because the angle between $\q_2$ and $-\g$ is smaller than that between $\q_3$ and $-\g$.

% Traditionally, boosting algorithms generates weak learners in each iteration, but the generated weak learners are not changed in the following iterations.
% However, in the context of rule ensemble learning, if the weights of a query is not changed, once the data points covered by this query are also covered by other queries generated later, the original weights cannot be optimal any more, although they are optimal when they are calculated.
% Therefore, to get a more accurate rule ensemble, we consider reweighting all the queries after a query is selected.

% To reweigh all the queries, we find a weight vector $\weights \in \R^t$ to minimize the empirical risk over $ \text{span}\{\textbf{q}_1,\cdots,\textbf{q}_t\}$, i.e.,
% \begin{equation}
%     \weights_t = \argmin_{\weights \in \R^t} R(\Q_t\weights)
%     \label{eq:weight_correction}
% \end{equation}
% where $\Q_t=[\q_1, \dots, \q_t]$ is the $n\times t$ \defemph{query matrix} with the output vectors of all selected queries as columns.
% \begin{equation}
%     \hat{R}(\textbf{w}^*)=\min_{\textbf{w}}{\hat{R}(\textbf{w})}.
% \end{equation}
% Given that our loss function $l$ and therefore the empirical risk $R$ are convex, solving this optimization problem is inexpensive relative to the overall computational complexity of the gradient boosting algorithm (especially when solving the single query optimization problem optimally via branch-and-bound). 
% In fact, the problem is equivalent to fitting one generalized linear model with $t$ input variables, which can be efficiently solved, e.g., with the Newton-Raphson algorithm (also referred to as \emph{iterated least squares} in this context).

% To get the minimum value of the empirical training risk, we can solve the equation
% \begin{equation}\label{eq:find_w}
%     \frac{\partial \hat{R}(\textbf{w})}{\partial \textbf{w}}=0.
% \end{equation}
% Here, Newton's method or Gradient descent method can be used to solve \eqref{eq:find_w}.


\subsection{An Objective Function to Identify the Best Approximating Subspace}

The intuitive reason for the gradient boosting objective failing to identify the correct query in Fig.~\ref{fig:subspace} is that selecting $x_2$ in addition to $x_3$ is not beneficial for the overall risk reduction \emph{if} we are only allowed to set the weight for the newly selected query. 
This is because then this weight has to be a compromise between the two different magnitudes of correction required for $x_2$, which only needs a small positive correction, and $x_3$, which needs a large positive correction.
If we, however, are allowed to change the weight of the previously selected query this consideration changes, because we can now balance an over-correction for $x_2$ by adjusting the weight of the first rule.
While on first glance it seems unclear how much of such re-balancing can be applied without harming the overall risk,
it turns out that this is captured by a simple criterion based on the norm of the part of the newly selected query that is orthogonal to the already selected ones.
\begin{lemma}\label{th:objective_func}
    For $\g\! \in \!\R^n$, $\Q\!=\![\q_1, \dots, \q_{t-1}] \in \R^{n \times (t-1)}$, and $\f\! \in \! \spanof\{\q_1, \dots, \q_{t-1}, \g\}$, we have
    \begin{equation}
        \argmin_{q \in \cQ} \min_{\weights \in \R^t} \|\f - [\q_1, \dots, \q_{t-1}, \q]\weights\|^2 = \argmax_{q \in \cQ} \frac{|\inner{\g_\perp}{\q}|}{\|\q_\perp\|} \enspace .
    \end{equation}
    where for a vector $\vecv \in \R^n$ we denote by $\vecv_\perp$ its projection onto the orthogonal complement of $\range \, \Q$. (All proofs of lemmas and theorems are in SI~\citep{github_url})
\end{lemma}
% \begin{proof}
%     Let $\f=[\Q; \g]\alpha$ and $\tilde{\f}=[\Q; q]\weights$. We can decompose the squared error
%     \begin{align*}
%         \|\f-\tilde{\f}\|^2 &= \|[\Q; \g]\alphavec - [\Q; \q]\weights\|^2\\
%         &=\|[\Q; \g_\parallel + \g_\perp]\alphavec - [\Q; \q_\parallel + \q_\perp]\weights\|^2\\
%         &=\|[\Q; \g_\parallel]\alphavec + \alpha_t\g_\perp - [\Q; \q_\parallel]\weights + \weight_t\q_\perp \|^2\\
%         &=\|[\Q; \g_\parallel]\alphavec - [\Q; \q_\parallel]\weights\|^2 + \|\alpha_t \g_\perp - \beta_t \q_\perp\|^2
%     \end{align*}
%     where the last step follows from the Pythagorean theorem and the fact that $\alpha_t \g_\perp - \beta_t \q_\perp$ is an element from the orthogonal complement of $\range [\Q; \g_\parallel]=\range[\Q; g_\parallel]=\range\, \Q$.
%     The equality of these ranges also implies that $\beta_1, \dots, \beta_{t-1}$ can, for all choices of $\beta_t$, be chosen such that the left term of the error decomposition is $0$. Setting $\gamma=\beta_t/\alpha_t$, it follows that
%     \begin{align*}
%         \min_{\weights \in \R^t} \|\f-\tilde{\f}\|^2 &= \min_{\beta \in \R^t} \|\alpha_t \g_\perp - \beta_t \h_\perp\|^2\\
%         &=\min_{\gamma \in \R^t} \alpha^2_t \|\g_\perp - \gamma \q_\perp\|^2\\
%         &=\min_{\gamma \in \R^t} \alpha_t^2 (\|\g_\perp\|^2-2\gamma \inner{\q_\perp}{\g_\perp} + \gamma^2\|\q_\perp\|^2) \\
%         \intertext{and plugging in the minimizing $\gamma=\inner{\q_\perp}{\g_\perp}/\|\q_\perp\|^2$ }
%         &=\alpha^2(\|\g_\perp\| - (\inner{\g_\perp}{\q_\perp})^2/\|\q_\perp\|^2) \enspace ,
%     \end{align*}
%     from which, noting that $\inner{\g_\perp}{\q_\perp}=\inner{\g_\perp}{\q}$, the claim follows.
% \end{proof}
From this result we can directly derive $|\inner{\g_\perp}{\q}|/\|\q_\perp\|$ as suitable objective function for fully corrective gradient boosting.
However, it is worth incorporating two further observations. 
Firstly, we can show that, after applying the weight correction step~\eqref{eq:weight_correction}, the gradient vector satisfies $\g=\g_\perp$, i.e., it is orthogonal to the subspace spanned by the selected queries, and therefore can be used in the objective function without projection.
\begin{lemma}
Let $\g$ be the gradient vector after the application of the weight correction step~\eqref{eq:weight_correction} for selected queries $\q_1, \dots, \q_t$. Then $\g \perp \spanof\{\q_1, \dots, \q_t\}$.
\label{th:g_orth}
\end{lemma}
% \begin{proof}
%     After the weight correction step $\weights$ is a stationary point of $R(\Q(\cdot))$, i.e., we have for all $j \in [t]$
%     \begin{equation*}
%         0 = \frac{\partial R(\Q\weights)}{\partial \beta_j}
%           = \sum_{i=1}^n \frac{\partial\, l(\inner{\tilde{\q}_i}{\weights}, y_i)}{\partial \beta_j} 
%           = \sum_{i=1}^n q_{ij} \underbrace{\frac{\partial\, l(\inner{\tilde{\q}_i}{\weights}, y_i)}{\partial\, \inner{\tilde{\q}_i}{\weights}}}_{g_i} = \inner{\q_j}{\g} \enspace .
%     \end{equation*}
% \end{proof}
Moreover, the right hand side of Eq.~\eqref{eq:gen_proj_error} is technically undefined for redundant query vectors $\q$ that lie in $\range\, \Q$ and therefore have $\|\q_\perp\|=0$.
Through Lm.~\ref{th:g_orth} we know that for such queries we also have $\inner{\g}{\q}=0$, which suggests to simply fix this issue by defining the objective value in this case to be $0$.
However, this solution would not fix numerical instabilities when $\|\q_\perp\|$ is close to zero.
A better solution is therefore to add a small positive value $\epsilon$ to the denominator, which can be considered a \defemph{regularization parameter}.
With this we arrive at the final form of our objective function, which we state along with some of its basic properties in the following theorem.
% (proof in SI~\citep{github_url}).
\begin{theorem}
Let $\Q = [\q_1, \dots, \q_{t-1}] \in \R^{n \times (t-1)}$ be the selected query matrix and $\g$ the corresponding gradient vector after full weight correction, and let us denote by $\q=\q_\perp+\q_\parallel$ the orthogonal decomposition of $\q$ with respect to $\range\, \Q$. 
%, and $\q^*$ a maximizer of the \defemph{orthogonal gradient boosting objective} 
% $
%     \ogbobj(q) = |\inner{\g}{\q}|/(\|\q_\perp\|+\epsilon)
% $
% where $\q_\perp$ is the projection of $\q$ onto the orthogonal complement of $\range \,\Q$. 
Then we have for a maximizer $\q^*$ of the \defemph{orthogonal gradient boosting objective} 
$
    \ogbobj(q) = |\inner{\g}{\q}|/(\|\q_\perp\|+\epsilon)
$:
\begin{itemize}
    \item[a)] For $\epsilon \to 0$, $\spanof\{\q_1, \dots, \q_{t-1}, \q^*\}$ is the best approximation to $\spanof\{\q_1, \dots, \q_{t-1}, \g\}$.
    % as defined in~\eqref{eq:gen_proj_error}.
    % \item[b)] For $\epsilon \to \infty$, $\q^*$ is a maximizer of $\gsobj$ and any maximizer of $\gsobj$ is a maximizer of $\ogbobj$.
    \item[b)] For $\epsilon \to \infty$, $\q^*$ maximizes $\gsobj$ and any maximizer of $\gsobj$ maximizes $\ogbobj$.
    \item[c)] For $\epsilon = 0$ and $\|\q_\perp\|>0$, the ratio $(\ogbobj(q)/\gbobj(q))^2$ is equal to $1+(\|\q_\parallel\|/\|\q_\perp\|)^2$.
    \item[d)] The objective value $\ogbobj(q)$ is upper bounded by $\|\g\|$.
\end{itemize}
    \label{thm:objective}
\end{theorem}
% \begin{comment}
% \begin{proof}
% %Pierre's attempt at proving b).
% Suppose that for $\epsilon \geq 0$, $q^* \in \argmax_q \ogbobj(q)$, and for any $q' \in \argmax_q \gsobj(q)$, we have $\frac{\gsobj(q')}{\|\q'_\perp\|+\epsilon} < \frac{\gsobj(q^*)}{\|\q^*_\perp\|+\epsilon}$.
% Then $\frac{\gsobj(q')}{\|\q'_\perp\|+\epsilon'} \geq \frac{\gsobj(q^*)}{\|\q^*_\perp\|+\epsilon'}$ if and only if $\epsilon' \geq \frac{\|\q'_\perp\|\gsobj(q^*) - \gsobj(q')\|\q^*_\perp\|}{\gsobj(q') - \gsobj(q^*)}$.
% Therefore, if $q^*$ is a maximizer of $\ogbobj$ for $\epsilon$, but not of $\gsobj$, there exists an $\epsilon'$ such that $q^*$ is not a maximizer of $\ogbobj$. We conclude that for large enough $\epsilon$, only maximizers of $\gsobj$ can be maximizers of $\ogbobj$.
% \end{proof}
% \end{comment}

% If there is a fully weight-correction step in each iteration of boosting, the weights of all rules are changed. However, the selected queries may not be the best after the weight-correction if the weight correction step is not considered during selection of queries. 

% Figure \ref{fig:subspace} shows two approximations to the subspace spanned by the existing query $\textbf{q}_1$ and the negative gradient vector $-\textbf{g}$. $\textbf{q}_2$ is more closed to $-\textbf{g}$ than $\textbf{q}_3$, and therefore it is preferred by the objective function \eqref{eq:gb_obj} of gradient boosting. However, the subspace $\text{span}\{\textbf{q}_1, \textbf{q}_3\}$ is more closed to $\text{span}\{\textbf{q}_1, \textbf{g}\}$ than $\text{span}\{\textbf{q}_1, \textbf{q}_2\}$.

% \begin{proposition} \label{th:gb_not_best}
% In the subspace of complete ensemble coefficients, the objective function of gradient boosting \eqref{eq:gb_obj} does NOT identify the best geometric approximation to the subspace spanned by existing queries and the gradient.
% \end{proposition}

% Proposition \ref{th:gb_not_best} indicates that we have to take into consideration the weight-correction step. Therefore, it requires a new objective function to select the most suitable queries.
% In this section, we introduce the novel objective function which is used in our approach.

% Figure \ref{fig:orth_demo} demonstrates the idea of the orthogonal projection in the proposed algorithm. 
% There are three data points in the 3-D space, and a rule $w_1q_1$ covering both $(x_1, y_1) $ and $(x_2, y_2)$ is learned already.  
% If there are two candidate queries, $q_2$ and $q_3$, as shown in the figure, and $q_2$ covers only one data point $(x_3, y_3)$, while $q_3$ covers both $(x_1, y_1)$ and $(x_3, y_3)$.
% Before the orthogonal projection, the query $q_2$ is more closed to the negative gradient vector $-\textbf{g}$ than $q_3$.
% However, if we have a fully-corrective step, actually the component of the candidate queries parallel to the subspace spanned by the existing rules does not affect the prediction. 
% Therefore, we can calculate the component of the queries which affect the output of the model by calculating the orthogonal projection of the queries. 
% (Here``orthogonal projection'' means the projection of the query onto the subspace orthogonal to all the existing rules.)
% We can see that the orthogonal projection of $q_2'$ is closer to the negative gradient vector $-\textbf{g}$ than the orthogonal projection of $q_2$. 


% If there are already $k$ rules learned, we define the query matrix across all the data points as \eqref{eq:query_matrix}:
% \begin{equation}\label{eq:query_matrix}
%     Q_k=\left[\textbf{q}_1,..., \textbf{q}_k\right], 
% \end{equation}
% where $\textbf{q}_i = [q_i(x_1), ... q_i(x_n)]^T$ is the output vector of the $i$th query.



% The projection of a query $\textbf{q}$ on the subspace orthogonal to the existing queries is calculated by \eqref{eq:orth_proj}:
% \begin{equation}\label{eq:orth_proj}
%     \textbf{q}_\bot=\left(I-Q_k(Q_k^TQ_k)^{-1}Q_k^T\right)\textbf{q}.
% \end{equation}
% The objective function is
% \begin{equation}\label{eq:orth_obj}
%     \text{obj}_{\text{orth}}(\textbf{q})=\frac{|\textbf{q}_\bot\cdot\textbf{g}|}{\norm{\textbf{q}_\bot}},
% \end{equation}
% where $$\textbf{g}=\left[\frac{\partial l(f(x_1), y_1)}{\partial f(x_1)}, \dots, \frac{\partial l(f(x_n), y_n)}{\partial f(x_n)}\right]^T.$$

Intuitively, the orthogonal gradient boosting objective function measures the cosine of the angle between the gradient vector and the orthogonal projection of a candidate query vector $\q$. This is in contrast to the standard gradient boosting objective, which considers the angle of the unprojected query vector instead. 
In the example in Fig.~\ref{fig:subspace} we can observe that this difference leads to successfully identifying the best approximating subspace, and
Thm.~\ref{thm:objective}a) guarantees this property.

\begin{algorithm}[tb]
   \caption{Fully-corrective Orthogonal Gradient Boosting}
   \label{alg:fcogb}
\begin{algorithmic}
   \STATE {\bfseries Input:} dataset $(x_i, y_i)_{i=1}^{n}$, desired number of rules $k$
   \STATE Initialise $f^{(0)}=0$
   \FOR{$t=1$ {\bfseries to} $k$}
   \STATE $\textbf{g}=\left(\frac{\partial l(f^{(t-1)}(x_1), y_1)}{\partial f^{(t-1)}(x_1)}, \dots, \frac{\partial l(f^{(t-1)}(x_n), y_n)}{\partial f^{(t-1)}(x_n)}\right)$
   \STATE $q_t=\argmax_{q \in \cQ}{\frac{|\inner{\q}{\g}|}{\|\q_\perp\|}}$ via \texttt{beam}($\g$, $\matO_{t-1}$) or \texttt{bb}($\g$, $\matO_{t-1}$)
   \STATE $\veco_t=\q_{t\perp}/\|\q_{t\perp}\|$ and $\matO_{t}=[\matO_{t-1}; \veco_t]$
   \STATE $\weights_t = \argmin_{\weights \in \R^t}{R([\q_1, \dots, \q_t]\weights)}$ via \texttt{convex\_opt}
   \STATE $f^{(t)}=[\q_1, \dots, \q_t]\weights_t$ %\left\{\textbf{q}^{(1)}_*, \dots, \textbf{q}^{(t)}_*\right\}\textbf{w}^{(t)}_*$
   \ENDFOR
   \STATE {\bfseries Output:} $f^{(k)}(\cdot)=\beta_{k, 1}q_1(\cdot)+\dots+\beta_{k, k}q_k(\cdot)$
\end{algorithmic}
\end{algorithm}

% Now we show that the objective function of the proposed algorithm identifies the subspace spanned by existing queries and the new query approximates best geometrically to the subspace spanned by existing queries and the gradient.
% \begin{theorem}
% The orthogonal objective function~\eqref{eq:orth_obj} identifies a vector $\hat{\textbf{q}}$ such that 
% for any vector $\textbf{v}^{(g)}\in\text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k, \textbf{g}\}$
% there exists a vector $\hat{\textbf{v}}\in\text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k, \hat{\textbf{q}}\}$ which satisfies
% \begin{equation*}
%     \norm{\textbf{v}^{(g)}-\hat{\textbf{v}}}=\min_{\textbf{q}}\left(\min_{\textbf{v}\in\text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k, \textbf{q}\}}\norm{\textbf{v}^{(g)}-\textbf{v}}\right).
% \end{equation*}
% \end{theorem}
% \begin{proof}
% For any vector \textbf{g} and $\textbf{q}$, they can be written as 
% $\textbf{g}=\textbf{g}_Q+\textbf{g}_\bot$
% and $\textbf{q}=\textbf{q}_Q+\textbf{q}_\bot, $ where $\textbf{g}_Q,\textbf{q}_Q \in \text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k\}, $
% and both $\textbf{g}_\bot$ and $\textbf{q}_\bot$ are in the subspace orthogonal to $\text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k\}$.

% Let $\textbf{v}^{(g)}=[Q^{(k)}; \textbf{g}]\textbf{w}^{(g)}$
% and $\textbf{v}^{(q)}=[Q^{(k)}; \textbf{q}]\textbf{w}^{(q)},$
% then
% \begin{align*}
%     &\norm{\textbf{v}^{(q)}-\textbf{v}^{(g)}}^2_2\\
%     =&\norm{[Q^{(k)}; \textbf{q}]\textbf{w}^{(q)}-[Q^{(k)}; \textbf{g}]\textbf{w}^{(g)}}_2^2\\
%     =&\norm{[Q^{(k)}; \textbf{q}_Q]\textbf{w}^{(q)}+w_{k+1}^{(q)}\textbf{q}_\perp-[Q^{(k)};\textbf{g}_Q] \textbf{w}^{(g)}-w_{k+1}^{(g)}\textbf{g}_\perp}_2^2\\
%     =&\norm{[Q^{(k)}; \textbf{q}_Q]\textbf{w}^{(q)}-[Q^{(k)};\textbf{g}_Q] \textbf{w}^{(g)}}_2^2+\\
%     &\norm{w_{k+1}^{(q)}\textbf{q}_\perp-w_{k+1}^{(g)}\textbf{g}_\perp}_2^2\\
% \end{align*}

% Since $\textbf{g}_Q,\textbf{q}_Q \in \text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k\},$ 
% these two vectors can be the same.
% Therefore, 
% \begin{align}\label{eq:min_diff_norm}
%     &\min\norm{\textbf{v}^{(q)}-\textbf{v}^{(g)}}_2^2\\
%     =&\min\norm{w_{k+1}^{(q)}\textbf{q}_\perp-w_{k+1}^{(g)}\textbf{g}_\bot}_2^2\\
%     \intertext{setting $\alpha=w_{k+1}^{(q)}/w_{k+1}^{(g)}$and $\gamma = w_{k+1}^{(g)}$}
%     =&\min\norm{\alpha\textbf{q}_\perp - \textbf{g}_\bot}_2^2 \gamma^2\\
%     =&\min\left(\textbf{g}_\bot\cdot\textbf{g}_\bot - 2\alpha\textbf{q}_{\perp}\cdot\textbf{g}_\bot+\alpha^2\textbf{q}_{\perp}\cdot\textbf{q}_\perp\right)\gamma^2 \\
%     \intertext{which is minimized for $\alpha=\textbf{q}_{\perp}\cdot\textbf{g}_\bot/\textbf{q}_{\perp}\cdot\textbf{q}_{\perp} $}=&\min\left(\textbf{g}_\bot\cdot\textbf{g}_\bot-\frac{\left(\textbf{q}_{\perp}\cdot\textbf{g}_\bot\right)^2}{\textbf{q}_{\perp}\cdot\textbf{q}_\perp}\right)\gamma^2,
% \end{align}
% Because of Lemma \ref{th:g_orth}, $\textbf{g}$ is always same as $\textbf{g}_\bot$.
% Therefore, maximising
% $
%     \cfrac{\left(\textbf{q}_{\perp}\cdot\textbf{g}\right)^2}{\norm{\textbf{q}_{\perp}}_2^2}
% $
% or 
% $
%     \cfrac{\left|\textbf{q}_{\perp}\cdot\textbf{g}\right|}{\norm{\textbf{q}_{\perp}}_2}
% $
% finds the vector $\hat{\textbf{q}}$ such that $\text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k, \hat{\textbf{q}}\}$
% best geometrically approximates
% $\text{span}\{\textbf{q}_1,\cdots,\textbf{q}_k, \textbf{g}\}$.

% \end{proof}

\input{4_1_table_updated.tex}
\subsection{Efficient Implementation}
%Having abstractly defined a rule objective function that is suitable in conjunction with full weight correction, we now turn to the question of how it can be computed efficiently in the context of the gradient boosting framework.
To develop an efficient optimization algorithm for the orthogonal gradient boosting objective, 
we recall that projections $\q_\perp$ on the orthogonal complement of $\range\,\Q$ can be naively computed via $\q_\perp=\Q((\Q^T\Q)^{-1}(\Q^T\q))$
% $
%     \q_\perp = \q - \underbrace{\Q((\Q^T\Q)^{-1}(\Q^T\q))}_{\q_\parallel}
% $
where we placed the parentheses to emphasize that only matrix-vector products are involved in the computation---at least once the inverse of the Gram matrix $\Q^T\Q$ is computed.
This approach allows to compute projections, and thus objective values, in time $O(nt+t^2)$ per candidate query after an initial preprocessing per boosting round of cost $O(t^2n + t^3)$.

%While the dependencies on $t$ might seem negligible 
In a first step, this naive approach can be improved by maintaining an orthonormal basis of the range of the query matrix throughout the boosting rounds, resulting in a Gram-Schmidt-type procedure. Since the projections $\q_{t \perp}$ of the selected queries naturally form an orthogonal basis of $\range\, \Q$ this only requires normalization, which can be done essentially without additional cost. Formally, by storing $\veco_t = \q_{t\perp} / \|\q_{t\perp}\|$ in all boosting rounds $t$, subsequent projections can be computed via
$
    q_\perp = \q - \matO(\matO^T\q)
    % \label{eq:proj_with_O}
$
where $\matO=[\veco_1, \dots, \veco_t]$.
This reduces the computational complexity per candidate query to $O(tn)$ without requiring any additional preprocessing.

While this looks like the optimal complexity for evaluating $\ogbobj$ in isolation, it leads to a prohibitive complexity for large $n$ for finding the optimal query in a given round.
Specifically, branch-and-bound with the tight bounding function~\eqref{eq:tight_bound} evaluates $O(n)$ queries per expanded search node  and beam search even $O(d^2n)$.
In both cases, using the expression for $\q_\perp$ above repeatedly results in a quadratic cost in $n$ per search node.
To circumvent this, we have to exploit the structure of candidate evaluations, similar to other efficient implementations of rule and tree learning algorithms~\citep{mampaey2015efficient}. 

The candidates evaluated per search node of both branch-and-bound and beam search have query vectors that are prefixes of an ordered sub-selection of data points, 
in beam search because optimum cut-off values are sought for each of the $d$ input variables,
in branch-and-bound because the optimum in Eq.~\eqref{eq:tight_bound} is attained or  approximated by a prefix with respect to some presorting order. 
% (e.g., based on $g_i$ for the gradient boosting objective or $g_i/h_i$ for the extreme gradient boosting objective.
Hence, we need to solve the following \defemph{prefix optimization problem}: given an ordered sub-selection of $l$ of the $n$ data points, represented by an injective map $\sigma\from \{1, \dots, l\} \to \{1, \dots, n\}$, find the optimal prefix 
\begin{equation}
 i_* = \argmax_{i \in \{1, \dots, l\}} \frac{\inner{\g}{\q^{(i)}}}{\|\q^{(i)}_\perp\| + \epsilon} 
 \label{eq:best_prefix}
\end{equation}
where $\q^{(0)}=\0$ and $\q^{(i)}=\q^{(i-1)}+\e_{\sigma(i)}$.
%A naive solution to this problem is to compute the projection matrix $\M=\I-\matO\matO^T \in \R^{n \times n}$ with $\matO=[\veco_1,\dots, \veco_t]$ and use it to compute the projection $\q^{(i)}_\perp = \M\q^{(i)}$ of all $i$ prefixes to find the maximum in Eq.~\eqref{eq:best_prefix}.
%While this approach is straightforward to implement, its computational complexity is of order $O(n^3)$, given that usually $l \approx n$, because it requires the computation of $l$ matrix-vector products involving an $n$-by-$n$ matrix. 
The following proof shows how the computational complexity for solving~\eqref{eq:best_prefix} can be substantially reduced compared to the direct approach above. 
It uses an incremental computation of projections that works directly on the available orthonormal basis vectors $\veco$ instead of computing matrix-vector products or, even worse, the whole projection matrix.
\begin{theorem}
    Given a gradient vector $\g \in \R^n$, an orthonormal basis $\veco_1, \dots, \veco_t \in \R^n$ of the subspace spanned by the queries of the first $t$ rules, and a sub-selection of $l$ candidate points $\sigma\from [l] \to [n]$, the best prefix selection problem~\eqref{eq:best_prefix} can be solved in time $O(tn)$.
    \label{thm:fast_prefix}
\end{theorem}
\begin{proof}[Proof sketch]
    We write the objective value of prefix $i$ in terms of incrementally computable quantities:
    \begin{equation*}
        \frac{\inner{\g}{\q^{(i)}}}{\|\q^{(i)}_\perp\| + \epsilon} = \frac{\inner{\g}{\q^{(i)}}}{\|\q^{(i)}\| - \|\q^{(i)}_\parallel\| + \epsilon} = \frac{\inner{\g}{\q^{(i)}}}{\|\q^{(i)}\| - \sqrt{\sum_{k=1}^t \|\veco_k \veco_k^T\q^{(i)}\|^2} + \epsilon}
        \enspace .
    \end{equation*}
    In particular, the $t$ sequences of norms $\|\veco_k \veco_k^T\q^{(i)}\|$ can be computed in time $O(n)$ via cumulative summation of the $k$-th basis vector elements in the order given by $\sigma$:
    \begin{align*}
        \|\veco_k\veco_k^T\q^{(i)}\|
        %=\left\|\veco_k\veco_k^T\left(\sum_{j=1}^i\e_{\sigma(j)}\right)\right\|
        =\|\veco_k\| \sum_{j=1}^i \inner{\veco_k}{\e_{\sigma(j)}}
        =\sum_{j=1}^i o_{k, \sigma(j)} 
    \end{align*}
    %To incrementally compute $\|q^{(i)}\|$  in time $O(t)$ per $i \in [n]$ as required by the claim we reduce the problem
\end{proof}
% \begin{proof}
%     To see the claim, we first rewrite the objective value for the $i$-th prefix as
%     \begin{equation*}
%         \frac{\inner{\g}{\q^{(i)}}}{\|\q^{(i)}_\perp\| + \epsilon} = \frac{\inner{\g}{\q^{(i)}}}{\|\q^{(i)}\| - \|\q^{(i)}_\parallel\| + \epsilon} 
%         \enspace .
%     \end{equation*}
%     The value of $\|\q^{(i)}\|$ is trivially given as $\sqrt{i}$, and $\inner{\g}{\q^{i}}$ can be easily computed for all $i \in [l]$ in time $O(n)$ via cumulative summation.
%     Finally we can reduce the problem of computing the (squared) norms of the $l$ projected prefixes to computing the $t$ (squared) norms of the prefixes on the subspaces given by the individual orthonormal basis vectors via
%     \begin{equation*}
%         \|\q^{(i)}_\parallel\|^2 = \left\|\sum_{k=1}^t \veco_k \veco_k^T\q^{(i)}\right\|^2 = \sum_{k=1}^t \|\veco_k \veco_k^T\q^{(i)}\|^2 \enspace .
%     \end{equation*}
%     Each of these $t$ sequences of (squared) norms can be computed in time $O(n)$ by rewriting
%     \begin{align*}
%         \|\veco_k\veco_k^T\q^{(i)}\| &= \left\|\veco_k\veco_k^T\left(\sum_{j=1}^i\e_{\sigma(j)}\right)\right\|\\
%         &=\|\veco_k\| \sum_{j=1}^i \inner{\veco_k}{\e_{\sigma(j)}}\\
%         &=\sum_{j=1}^i o_{k, \sigma(j)} 
%     \end{align*}
%     where the last equality shows how an $O(n)$-computation is achieved via cumulative summation of the $k$-th basis vector elements in the order given by $\sigma$.
%     %To incrementally compute $\|q^{(i)}\|$  in time $O(t)$ per $i \in [n]$ as required by the claim we reduce the problem
% \end{proof}
We close this section with a pseudocode (Alg.~\ref{alg:fcogb}) that summarizes the main ideas of the orthogonal gradient boosting and refer to the literature for details about the beam-search/branch-and-bound step.

% To find the query which maximise the objective function, a branch-and-bound approach proposed by \citet{boley2021better} is adopted.
% According to Lemma \ref{th:g_orth}, $\inner{\g}{\q_Q}=0,$ so $\inner{\g}{\q_\bot}=\inner{\g}{\q}$. 
% Let $I(\q)$ represent the support set of $\q$, then

% If there is a fully weight-correction step in each iteration of boosting:

% \begin{align}
%     \text{bnd}(\textbf{q})=\max_{J\subseteq I(\q)}\frac{\max\sum_{i\in J}{g_i}}{\min\left\{\norm{\q'_\bot}_2:\norm{\q'}_1=|J|, I(\q')\subseteq I(\q)\right\}}.
% \end{align}

% \subsection{Orthogonal projection approach covers more data points}
% Theorem \ref{th:more_parallel} shows that with the orthogonal projection approach, the selected queries tend to select more data points covered by previous rules than the approach without orthogonal projection.
% \begin{lemma}\label{th:more_parallel}
% If
% \begin{equation}\label{eq:orth_obj_max}
%     \textbf{u}=\arg\max_{\textbf{q}}\frac{|\textbf{q}_\perp\cdot\textbf{g}|}{||\textbf{q}_\perp||}, 
% \end{equation}
% and 
% \begin{equation}\label{eq:gpe_obj_max}
%     \textbf{v}=\arg\max_{\textbf{q}}\frac{|\textbf{q}\cdot\textbf{g}|}{||\textbf{q}||},
% \end{equation}
% then
% \begin{equation}
%     \frac{||\textbf{v}_\perp||}{||\textbf{v}_{\mathbin{\!/\mkern-5mu/\!}} ||}\geq\frac{||\textbf{u}_\perp||}{||\textbf{u}_{\mathbin{\!/\mkern-5mu/\!}} ||}.
% \end{equation}
% \end{lemma}
% \begin{proof}

% From \eqref{eq:orth_obj_max}, we get
% \begin{equation}
% \frac{\left|\textbf{u}_\perp\cdot\textbf{g}\right|}{||\textbf{u}_\perp||}\geq\frac{\left|\textbf{v}_\perp\cdot\textbf{g}\right|}{||\textbf{v}_\perp||},
% \end{equation}
% which means 
% \begin{equation}
%     \frac{\left|\textbf{u}_\perp\cdot\textbf{g}\right|}{\left|\textbf{v}_\perp\cdot\textbf{g}\right|}\geq\frac{||\textbf{u}_\perp||}{||\textbf{v}_\perp||}.
% \end{equation}
% From \eqref{eq:gpe_obj_max}, we get
% \begin{equation}
% \frac{\left|\textbf{v}\cdot\textbf{g}\right|}{\sqrt{||\textbf{v}_\perp||^2+||\textbf{v}_{\mathbin{\!/\mkern-5mu/\!}}||^2}}=
%     \frac{\left|\textbf{v}\cdot\textbf{g}\right|}{||\textbf{v}||}\geq\frac{\left|\textbf{u}\cdot\textbf{g}\right|}{||\textbf{u}||}
%     =\frac{\left|\textbf{u}\cdot\textbf{g}\right|}{\sqrt{||\textbf{u}_\perp||^2+||\textbf{u}_{\mathbin{\!/\mkern-5mu/\!}}||^2}},
% \end{equation}
% which means
% \begin{equation}
%     \frac{\sqrt{||\textbf{u}_\perp||^2+||\textbf{u}_{\mathbin{\!/\mkern-5mu/\!}}||^2}}{\sqrt{||\textbf{v}_\perp||^2+||\textbf{v}_{\mathbin{\!/\mkern-5mu/\!}}||^2}}
%     \geq\frac{\left|\textbf{u}\cdot\textbf{g}\right|}{\left|\textbf{v}\cdot\textbf{g}\right|}
% \end{equation}
% From Lemma \ref{th:g_orth} and Lemma \ref{th:eq_span}, we know
% \begin{equation}
%     \textbf{u}_{\mathbin{\!/\mkern-5mu/\!}}\cdot\textbf{g}=\textbf{v}_{\mathbin{\!/\mkern-5mu/\!}}\cdot\textbf{g}=0.
% \end{equation}
% Therefore,
% \begin{equation}
%     \textbf{u}\cdot\textbf{g}=\textbf{u}_\perp\cdot\textbf{g}+\textbf{u}_{\mathbin{\!/\mkern-5mu/\!}}\cdot\textbf{g}=\textbf{u}_\perp\cdot\textbf{g}.
% \end{equation}

% In the end, we can conclude that
% \begin{equation*}
%     % ||\textbf{u}_{\mathbin{\!/\mkern-5mu/\!}}||\geq||\textbf{v}_{\mathbin{\!/\mkern-5mu/\!}} ||?
%     \frac{||\textbf{v}_\perp||}{||\textbf{v}_{\mathbin{\!/\mkern-5mu/\!}} ||}\geq\frac{||\textbf{u}_\perp||}{||\textbf{u}_{\mathbin{\!/\mkern-5mu/\!}} ||}
% \end{equation*}

% \end{proof}


==> old/4_1_table.tex <==
\begin{table}
\caption{Comparison of normalised training risks and computation times for rule ensembles, averaged over cognitive complexities between 1 and 50, using SIRUS(SRS), Gradient Sum(GS), Gradient boosting (GB), XGBoost (XGB) and FCOGB, for benchmark datasets of classification (upper), regression (middle) and Poisson regression problems (lower).}
\label{tb:comparison}
\vskip 0.05in
% \hskip 0.05in
\begin{center}
\begin{scriptsize}
\begin{sc}
\begin{comment}
    
\begin{tabular}{l@{\hskip 0.05in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}c@{\hskip 0.05in}r}
% \begin{tabular}{lcccccccccccccccr}
\toprule
% dataset &feat&row&$\bar{\Delta}_\mathrm{GO}$ & $\bar{\Delta}_\mathrm{XO}$ & $\Delta_\mathrm{GO}^\mathrm{bc}$& $\Delta_\mathrm{XO}^\mathrm{bc}$ & $\Delta_\mathrm{GO}^\mathrm{wc}$ & $\Delta_\mathrm{XO}^\mathrm{wc}$ & $\bar{\Tilde{R}}_\mathrm{O}$ & $c_\mathrm{GO}^\mathrm{bc}$ & $c_\mathrm{XO}^\mathrm{bc}$ & $c_\mathrm{GO}^\mathrm{wc}$ & $c_\mathrm{XO}^\mathrm{wc}$ &$\text{T}_\mathrm{G}^{(10)}$&$\text{T}_\mathrm{X}^{(10)}$&$\text{T}_\mathrm{O}^{(10)}$\\
\multirow{2}{*}{dataset} & \multirow{2}{*}{$d$} & \multirow{2}{*}{$n$} & \multirow{2}{*}{$\bar{\Tilde{R}}_\mathrm{O}$} & \multicolumn{5}{c}{FCOGB vs. GS} & \multicolumn{5}{c}{FCOGB vs. GB} & \multicolumn{5}{c}{FCOGB vs XGBoost} & \multicolumn{1}{c}{\multirow{2}{*}{$\text{T}_\mathrm{S}^{(10)}$}} & \multirow{2}{*}{$\text{T}_\mathrm{G}^{(10)}$} & \multirow{2}{*}{$\text{T}_\mathrm{X}^{(10)}$} & \multirow{2}{*}{$\text{T}_\mathrm{O}^{(10)}$} \\
 &  &  &  & \multicolumn{2}{c}{$\Delta_\mathrm{SO}^\mathrm{bc}$} & \multicolumn{1}{c}{$\bar{\Delta}_\mathrm{SO}$} & \multicolumn{2}{c}{$\Delta_\mathrm{SO}^\mathrm{wc}$} & \multicolumn{2}{c}{$\Delta_\mathrm{GO}^\mathrm{bc}$} & $\bar{\Delta}_\mathrm{GO}$ & \multicolumn{2}{c}{$\Delta_\mathrm{GO}^\mathrm{wc}$} & \multicolumn{2}{c}{$\Delta_\mathrm{XO}^\mathrm{bc}$} & $\bar{\Delta}_\mathrm{XO}$ & \multicolumn{2}{c}{$\Delta_\mathrm{XO}^\mathrm{wc}$} & \multicolumn{1}{c}{} &  &  &  \\


\midrule
titanic & 7 & 1043 & .658 & .076 & (22.6) & .043 & .000 & (2.4) & .122 & (5.2) & .017 & -.030 & (7.4) & .131 & (5.2) & .031 & -.021 & (4.4) & 1.660 & 20.87 & 26.81 & 26.44\\
tic-tac-toe & 27 & 958 & .656 & .308 & (27.4) & .149 & -.072 & (1.4) & .137 & (29.4) & .037 & -.001 & (6.2) & .204 & (29.4) & .085 & .002 & (2.4) & 5.570 & 29.29 & 23.06 & 47.68\\
iris & 4 & 150 & .317 & .397 & (5.8) & .041 & -.028 & (7.2) & .268 & (5.8) & .027 & -.102 & (3.6) & .327 & (5.8) & .094 & -.044 & (3.6) & .785 & 2.010 & 2.075 & 2.090\\
breast & 30 & 569 & .358 & .027 & (7.8) & -.011 & -.236 & (7) & .037 & (32.4) & .003 & .000 & (2.4) & .085 & (7.8) & .041 & .005 & (10.4) & 8.505 & 116.2 & 177.8 & 257.3\\
wine & 13 & 178 & .241 & .326 & (2.4) & .045 & -.279 & (5.8) & .318 & (6) & .062 & -.123 & (3.8) & .380 & (6) & .110 & -.061 & (3.8) & 2.015 & 7.713 & 1.151 & 30.09\\
ibm hr & 32 & 1470 & .212 & .022 & (5.6) & .003 & .000 & (11.8) & .029 & (5.6) & .003 & -.002 & (17.8) & .049 & (5.6) & .008 & .004 & (22) & 15.67 & 7.488 & 20.25 & 11.44\\
telco churn & 18 & 7043 & .695 & .062 & (2.4) & .012 & -.166 & (1.4) & .054 & (9.4) & .018 & -.006 & (12.4) & .027 & (15.4) & .008 & -.009 & (12.4) & 22.45 & 5266 & 5190 & 5343\\
gender & 20 & 3168 & .997 & .002 & (2.4) & .000 & .000 & (3.2) & .000 & (2.4) & .000 & .000 & (18.4) & .000 & (16.4) & .000 & .000 & (11.4) & 6.543 & 42.66 & 32.38 & 28.47\\
banknote & 4 & 1372 & .337 & .108 & (19.6) & .056 & -.046 & (8.2) & .113 & (15.2) & .017 & .000 & (5.2) & .110 & (19.6) & .057 & -.024 & (9.4) & 6.492 & 10.08 & 13.83 & 6.991\\
liver & 6 & 345 & .837 & .072 & (28.8) & .019 & -.059 & (9.2) & .053 & (15.2) & -.004 & -.052 & (22) & .068 & (56.4) & .004 & -.030 & (20) & 2.015 & 145.2 & 301.4 & 234.5\\
magic & 10 & 19020 & .731 & .042 & (8.2) & .013 & -.031 & (4.2) & .003 & (8.2) & -.002 & -.015 & (13.4) & .019 & (18.4) & .005 & -.004 & (13.4) & 73.11 & 71.10 & 194.2 & 138.9\\
adult & 11 & 30162 & .608 & .151 & (2.4) & .012 & -.190 & (1.4) & .049 & (10.4) & .018 & .000 & (2.4) & .067 & (4.2) & .012 & .001 & (5.2) & 100.9 & 392.0 & 381.7 & 347.5\\
digits5 & 64 & 3915 & .393 & .026 & (4.2) & .017 & -.028 & (3.2) & .031 & (10.4) & -.008 & -.044 & (23.4) & .062 & (4.2) & -.008 & -.038 & (19.4) & 60.38 & 110.7 & 37.98 & 125.8\\
\midrule
insurance & 6 & 1338 & .166 & .129 & (4.2) & .025 & -.540 & (1.4) & .186 & (4.2) & .026 & .000 & (2.4) & .186 & (4.2) & .026 & .000 & (2.4) & 10.90 & 19.50 & 37.62 & 28.48\\
friedman1 & 10 & 2000 & .080 & .017 & (4) & .000 & -.013 & (3.2) & .030 & (4) & .005 & .000 & (1.4) & .030 & (4) & .005 & .000 & (1.4) & 2.795 & 5.347 & 12.38 & 6.220\\
friedman2 & 4 & 10000 & .149 & .159 & (3.2) & -.023 & -.622 & (1.4) & .078 & (8.2) & .016 & -.066 & (5.2) & .078 & (8.2) & .016 & -.066 & (5.2) & 22.89 & 19.723 & 30.60 & 12.65\\
friedman3 & 4 & 5000 & .057 & .009 & (4.6) & .004 & -.011 & (4) & .020 & (4.6) & .002 & .000 & (1.4) & .020 & (4.6) & .002 & .000 & (1.4) & 8.313 & 12.766 & 27.42 & 12.37\\
wage & 5 & 1379 & .381 & .046 & (6.6) & .015 & -.051 & (4.6) & .097 & (6.6) & .013 & .000 & (1.4) & .097 & (6.6) & .013 & .000 & (1.4) & 9.077 & 21.263 & 29.60 & 20.64\\
demographics & 13 & 6876 & .225 & .010 & (5.2) & .004 & .000 & (1.4) & .007 & (3.2) & .002 & .000 & (1.4) & .007 & (3.2) & .002 & .000 & (1.4) & 36.37 & 21.707 & 49.56 & 30.39\\
gdp & 1 & 35 & .037 & .004 & (3.2) & .000 & .000 & (5.2) & .003 & (3.2) & .000 & .000 & (5.2) & .003 & (3.2) & .000 & .000 & (5.2) & .086 & .263 & .429 & .351\\
used cars & 4 & 1770 & .191 & .165 & (3.2) & -.020 & -.566 & (1.4) & .095 & (8.8) & .033 & .000 & (3.2) & .095 & (8.8) & .033 & .000 & (3.2) & 13.23 & 17.40 & 34.90 & 12.46\\
diabetes & 10 & 442 & .153 & .034 & (4.4) & .004 & -.032 & (3.4) & .065 & (4.4) & .007 & .000 & (1.4) & .065 & (4.4) & .007 & .000 & (1.4) & 2.598 & 5.813 & 8.926 & 7.529\\
boston & 13 & 506 & .103 & .030 & (4.4) & .007 & -.037 & (3.8) & .067 & (4.4) & .007 & -.009 & (9.2) & .067 & (4.4) & .007 & -.009 & (9.2) & 3.942 & 8.186 & 16.226 & 8.591\\
happiness & 8 & 315 & .047 & .011 & (5.2) & .001 & -.013 & (3.8) & .024 & (5.2) & .003 & .000 & (9.6) & .024 & (5.2) & .003 & .000 & (9.6) & .561 & 13.79 & 26.37 & 24.02\\
life expect. & 21 & 1649 & .040 & .003 & (4.2) & .000 & .000 & (8.2) & .009 & (4.2) & .001 & .000 & (10.4) & .009 & (4.2) & .001 & .000 & (10.4) & 20.28 & 55.46 & 144.6 & 150.6\\
mobile prices & 20 & 2000 & .163 & .196 & (2.4) & -.006 & -.642 & (1.4) & .045 & (3.2) & .003 & .000 & (4.2) & .045 & (3.2) & .003 & .000 & (4.2) & 21.67 & 775.4 & 1736 & 1101\\
suicide rate & 5 & 27820 & .553 & .077 & (2.4) & .020 & -.309 & (1.4) & .023 & (11.4) & .009 & .000 & (2.4) & .023 & (11.4) & .009 & .000 & (2.4) & 74.23 & 161.1 & 45.59 & 178.8\\
videogame & 6 & 16327 & .954 & .000 & (3.2) & .000 & .000 & (1.4) & .000 & (3.2) & .000 & .000 & (1.4) & .000 & (3.2) & .000 & .000 & (1.4) & 20.21 & 58.91 & 14.21 & 37.72\\
red wine & 11 & 1599 & .048 & .002 & (4.2) & .000 & -.002 & (3.2) & .001 & (4.2) & .000 & -.001 & (6.2) & .001 & (4.2) & .000 & -.001 & (6.2) & 3.736 & 30.03 & 17.72 & 37.25\\
\midrule
covid vic & 4 & 85 & .178 & .102 & (3) & .023 & -.061 & (10) & .083 & (10.6) & .014 & -.041 & (5.2) & 3.491 & (3) & .401 & .019 & (25.8) & .580 & .729 & 1.502 & .587\\
covid & 2 & 225 & .408 & .091 & (6.8) & -.023 & -.460 & (2) & .024 & (34.6) & .010 & -.013 & (10.4) & 19.978 & (6.8) & 3.857 & .230 & (24.2) & 1.032 & 1.026 & 2.153 & .832\\
bicycle & 4 & 122 & .401 & .165 & (7.8) & .034 & -.327 & (3.4) & .056 & (12.2) & .004 & -.003 & (36.4) & .035 & (7.8) & .011 & -.033 & (11.2) & .792 & 1.897 & 3.536 & 1.768\\
ships & 4 & 34 & .223 & .195 & (3.2) & -.011 & -.539 & (2.4) & .061 & (23.2) & .032 & -.008 & (10.6) & 796.7 & (3.2) & 145.0 & .249 & (29.6) & .265 & .367 & .597 & .362\\
smoking & 2 & 36 & .142 & .241 & (4.2) & .028 & -.025 & (6.6) & .050 & (7) & .013 & -.028 & (4.2) & 1.032 & (2.4) & .113 & .017 & (21.6) & .191 & .341 & .484 & .205\\
\bottomrule
\end{tabular}
\end{comment}
\begin{tabular}{l@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c}
\toprule
 &  &  & \multicolumn{5}{c}{Training Risks} & \multicolumn{5}{c}{Testing Risks} & \multicolumn{5}{c}{Computation Times} \\
\multirow{-2}{*}{Dataset} & \multirow{-2}{*}{$d$} & \multirow{-2}{*}{$n$} & SRS & GS & GB & XGB & FCOGB & SRS & GS & GB & XGB & FCOGB & SRS & GS & GB & XGB & FCOGB \\ \hline
titanic & 7 & 1043 & .895 & .662 & .635 & .637 & \textbf{.610} & .894 & .723 & .712 & .721 & \textbf{.707} & 7.077 & 2.624 & 9.858 & 10.21 & 25.71 \\
tic-tac-toe & 27 & 958 & .892 & .741 & .627 & .640 & \textbf{.587} & .885 & .800 & .722 & .689 & \textbf{.669} & 12.59 & 3.971 & 10.34 & 6.09 & 13.99 \\
iris & 4 & 150 & .685 & .253 & .222 & .287 & \textbf{.218} & .745 & \textbf{.384} & .429 & .408 & .511 & 11.02 & 0.775 & 1.099 & 1.453 & 2.487 \\
breast & 30 & 569 & .569 & \textbf{.273} & .291 & .314 & .292 & .627 & \textbf{.273} & .370 & .376 & .348 & 11.48 & 6.744 & 74.43 & 74.83 & 239.2 \\
wine & 13 & 178 & .578 & .162 & .216 & .192 & \textbf{.146} & .621 & .340 & .471 & .402 & \textbf{.242} & 9.456 & 1.530 & 4.432 & 2.154 & 55.18 \\
ibm hr & 32 & 1470 & .980 & .572 & .560 & .573 & \textbf{.560} & .974 & .607 & .618 & .626 & \textbf{.606} & 11.15 & 17.24 & 10.99 & 12.92 & 12.03 \\
telco churn & 18 & 7043 & .944 & .679 & .683 & .679 & \textbf{.670} & .945 & .663 & .677 & .673 & \textbf{.663} & 50.83 & 40.01 & 1883 & 1485 & 3039 \\
gender & 20 & 3168 & \textbf{.566} & .996 & .996 & .996 & .996 & \textbf{.570} & 1.000 & 1.000 & 1.000 & 1.000 & 22.42 & 22.73 & 25.49 & 24.27 & 32.95 \\
banknote & 4 & 1372 & .854 & .303 & .264 & .288 & \textbf{.227} & .858 & .310 & .263 & .297 & \textbf{.228} & 8.933 & 6.298 & 5.648 & 7.060 & 8.444 \\
liver & 6 & 345 & .908 & .809 & .800 & .787 & \textbf{.777} & .917 & \textbf{.913} & 1.000 & .928 & 1.000 & 9.734 & 1.997 & 99.72 & 124.1 & 193.9 \\
magic & 10 & 19020 & .906 & .720 & .709 & .710 & \textbf{.707} & .903 & .702 & .693 & .693 & \textbf{.687} & 1.364 & 75.14 & 89.18 & 101.9 & 352.2 \\
adult & 11 & 30162 & .804 & .594 & .599 & .594 & \textbf{.582} & .802 & .603 & .615 & .607 & \textbf{.597} & 2.169 & 121.0 & 136.7 & 146.0 & 728.3 \\
digits5 & 64 & 3915 & \textbf{.248} & .331 & .312 & .335 & .353 & \textbf{.262} & .329 & .314 & .330 & .350 & 52.60 & 110.8 & 72.74 & 101.5 & 97.4 \\ \hline
insurance & 6 & 1338 & .169 & .144 & .143 & .146 & \textbf{.126} & .177 & .134 & .137 & .140 & \textbf{.126} & 14.06 & 7.507 & 15.94 & 12.98 & 39.53 \\
friedman1 & 10 & 2000 & .180 & .069 & .073 & .071 & \textbf{.068} & .165 & \textbf{.072} & .080 & .079 & .074 & 16.79 & 2.514 & 4.302 & 3.171 & 6.915 \\
friedman2 & 4 & 10000 & \textbf{.082} & .092 & .119 & .116 & .101 & \textbf{.082} & .094 & .120 & .117 & .101 & 47.33 & 11.79 & 17.56 & 13.18 & 28.4 \\
friedman3 & 4 & 5000 & .093 & .044 & .043 & .043 & \textbf{.041} & .092 & .046 & .046 & .046 & \textbf{.044} & 29.86 & 6.243 & 10.61 & 8.559 & 17.65 \\
wage & 5 & 1379 & .427 & .368 & .366 & .355 & \textbf{.342} & \textbf{.341} & .377 & .397 & .394 & .396 & 14.18 & 5.605 & 12.12 & 13.17 & 25.19 \\
demographics & 13 & 6876 & .219 & .214 & .213 & .213 & \textbf{.212} & \textbf{.209} & .217 & .217 & .217 & .216 & 38.24 & 36.80 & 29.40 & 33.04 & 72.42 \\
gdp & 1 & 35 & .063 & .024 & .024 & .024 & \textbf{.024} & .059 & .025 & .025 & .025 & \textbf{.025} & 7.974 & .261 & .351 & .282 & .488 \\
used cars & 4 & 1770 & .373 & .266 & .250 & .251 & \textbf{.225} & .427 & .289 & .265 & .271 & \textbf{.241} & 15.00 & 8.371 & 12.10 & 9.484 & 20.27 \\
diabetes & 10 & 442 & .156 & .137 & .137 & .136 & \textbf{.130} & .188 & \textbf{.148} & .150 & .155 & .158 & 10.50 & 2.204 & 3.574 & 3.920 & 7.591 \\
boston & 13 & 506 & .101 & .089 & .090 & .087 & \textbf{.081} & .105 & \textbf{.078} & .086 & .086 & .081 & 10.96 & 3.055 & 6.731 & 5.285 & 10.44 \\
happiness & 8 & 315 & .109 & .031 & .031 & .032 & \textbf{.030} & .109 & \textbf{.033} & .038 & .038 & .037 & 6.344 & 1.160 & 11.37 & 11.31 & 26.43 \\
life expect. & 21 & 1649 & .109 & .026 & .026 & .026 & \textbf{.025} & .110 & .027 & .027 & .027 & \textbf{.026} & 21.44 & 16.16 & 58.43 & 63.82 & 131.2 \\
mobile prices & 20 & 2000 & .148 & \textbf{.131} & .137 & .137 & .135 & .140 & .136 & .143 & .145 & .142 & 33.81 & 15.03 & 367.7 & 442.5 & 815.4 \\
suicide rate & 5 & 27820 & .547 & .543 & .540 & .541 & \textbf{.534} & \textbf{.514} & .521 & .521 & .521 & .515 & 52.35 & 109.6 & 117.1 & 139.6 & 644.6 \\
videogame & 6 & 16327 & \textbf{.895} & .953 & .953 & .953 & .953 & .850 & .720 & .720 & .720 & \textbf{.720} & 1.171 & 41.91 & 34.38 & 45.90 & 119.1 \\
red wine & 11 & 1599 & .072 & .034 & .035 & .035 & \textbf{.034} & .073 & .035 & .035 & .036 & \textbf{.035} & 19.94 & 9.149 & 15.32 & 21.99 & 35.34 \\ \hline
covid vic & 4 & 85 & NA & .144 & .130 & .368 & \textbf{.125} & NA & .152 & \textbf{.127} & .382 & .130 & NA & .523 & .600 & .628 & .854 \\
covid & 2 & 225 & NA & \textbf{.341} & .374 & 2.893 & .347 & NA & \textbf{.447} & .482 &  4.115 & .469 & NA & .701 & .690 & .682 & 1.143 \\
bicycle & 4 & 122 & NA & .352 & .317 & .310 & \textbf{.300} & NA & \textbf{.413} & .439 & .440 & .467 & NA & .695 & 1.103 & 1.105 & 2.124 \\
ships & 4 & 34 & NA & .155 & .168 &  87.31 & \textbf{.145} & NA & \textbf{.222} & .288 & 109.1 & .420 & NA & .235 & .296 & .311 & .448 \\
smoking & 2 & 36 & NA & .114 & .109 & .165 & \textbf{.090} & NA & \textbf{.130} & .193 & .258 & .169 & NA & .266 & .256 & .208 & .301\\
\bottomrule
\end{tabular}
\end{sc}
\end{scriptsize}
\end{center}
\vskip -0.2in
\end{table}


==> old/4_experiments.tex <==
\section{Experiments}\label{experiments}
In this section, we present empirical results comparing the proposed fully corrective orthogonal gradient boosting (FCOGB) to the standard gradient boosting algorithms~\citep{dembczynski2010ender} using greedy optimization of $\gbobj$ (GB) and $\gsobj$ (GS), to extreme gradient booosting~\citep{boley2021better} using branch-and-bound optimisation of $\xgbobj$ (XGB), and finally to SIRUS \citep{benard2021interpretable} as the state-of-the-art generate-and-filter approach.
%Specifically, for the high-level comparison we consider FCOGB with branch-and-bound rule optimization with the bounding function based on gradient-based presorting, and, as alternatives the two algorithm presented in~\citet{dembczynski2010ender}, i.e., using $\gsobj$ and $\gbobj$ in conjunction with greedy optimization, as well the algorithm from~\citet{boley2021better}, i.e., using $\xgbobj$ in conjunction with branch-and-bound search.
% Additionally, we report on an ablation study were individual components of the algorithms are varied.
We investigate the risk/complexity trade-off, the affinity to select general rules, as well as the computational complexity.
The datasets used are those of \citet{boley2021better} augmented by three additional classification datasets from the UCI machine learning repository and, to introduce a novel modelling task to the rule learning literature, five counting regression datasets from public sources. 
This results in a total of 34 datasets (13 for classification, 16 for regression, and 5 for counting/Poisson regression, see Tab.~\ref{tb:comparison}).
All algorithms were run five times on all datasets using 5 random 80/20 train/test splits to calculate robust estimates of all considered metrics. 
In all cases, the number of gradient boosting iterations was chosen to produce ensembles with cognitive complexity of at most 50.
% which was used as a target value because it corresponds to a model size that humans can credibly comprehend.
The experiment code and further information about the datasets are available on GitHub\cite{github_url}.

% We run the experiments and compare the cognitive complexities, risks, coverages of each rule and computation times using the gradient sum approach, gradient boosting, XGBoost and FCOGB.
% For each dataset, we run the experiments on 5 random 80/20 training/testing splits. 
% After that, the average values of each benchmark for each dataset are calculated.
\begin{comment}
    
\begin{figure*}[t!]
\vskip 0.1in
\centering
\begin{center}
\includegraphics[width=\columnwidth]{Images/ablation_study_new.pdf}
\end{center}
\vskip -0.1in
\caption{The comparison of the risks of Gradient boosting, Fully-corrective boosting, Greedy FCOGB and optimal FCOGB. Each point in these figures represents the comparison of the risk of models generated by algorithms on the axis labels of one dataset. }
\label{fig:ablation_study}
\end{figure*}
\end{comment}

\paragraph{Cognitive complexity versus risk}
Tab.~\ref{tb:comparison} compares the complexity/risk trade-off of the boosting variants and SIRUS 
%by summarizing the trade-off curves (as visualized in Fig.~\ref{fig:compare_tic}) 
by the normalized risk averaged across all considered cognitive complexity levels (where normalization is performed by the risk of the empty rule ensemble).
FCOGB has the smallest training risk for 26 of the 34 datasets, occasionally outperforming the second best algorithm by a wide margin (\textit{tic-tac-toe}, \textit{wine}, \textit{banknote}, \textit{insurance}, \textit{boston}, \textit{ships},  \textit{smoking}).
For the test risk the picture is more ambiguous, however, FCOGB retains a relative majority of datasets won.
%In more detail, we consider the normalized risk value $\Tilde{R}(c)=R(c)/R(0)$ achieved by a method at complexity level $c$ where $R(0)$ specifically is the risk for the empty rule ensemble.
%Tab.~\ref{tb:comparison} compares the normalized risk of SIRUS, gradient sum, gradient boosting, XGBoost and FCOGB.
% a cognitive complexity level $c$ is
% \begin{equation}
%     \Tilde{R}(c) = \frac{\hat{R}(c)}{\hat{R}(0)},
% \end{equation}
% where $\hat{R}(0)$ is the empirical risk of zero-ensemble. Therefore, the maximum value of the normalised empirical risk is 1.
%
% Then we define the risk difference from algorithm A to algorithm B at complexity level $c$ as
% \begin{equation*}
%     \Delta_{\text{AB}}(c)=\Tilde{R}_\text{A}(c)-\Tilde{R}_\text{B}(c).
% \end{equation*}
% and consider the average, minimum, and maximum difference of this metric across $c \in \{1, \dots, 30\}$.
%
% Given a minimum value $c_{min}$ and a maximum value $c_{max}$ of the cognitive complexity level, the average risk difference of algorithm A comparing to algorithm B is
% \begin{equation}
%     \bar{\Delta}_\mathrm{AB}=\frac{1}{c_\mathrm{max}-c_\mathrm{min}}\sum_{c=c_\mathrm{min}}^{c_\mathrm{max}}{\Delta_\mathrm{AB}(c)}.
% \end{equation}
% We also define the difference of algorithm A over algorithm B in the worst (resp. best) case as
% \begin{equation}
%     \Delta_\mathrm{AB}^{wc}=\min\{\Delta_\mathrm{AB}(c): c_\mathrm{min}\leq c \leq c_\mathrm{max}\}
% \end{equation}
% and 
% \begin{equation}
%     \Delta_\mathrm{AB}^\mathrm{bc}=\max\{\Delta_\mathrm{AB}(c): c_\mathrm{min}\leq c \leq c_\mathrm{max}\},
% \end{equation}
% and the cognitive complexity at the worst (resp. best) case is written as $c_\mathrm{AB}^\mathrm{wc}$ (resp. $c_\mathrm{AB}^\mathrm{bc}$).
%
% The left portion (orange framed) of Fig.~\ref{fig:ablation_study} presents a summary of the results. 
% We can see that FCOGB has typically strongly reduced risk values at the most favourable (best case) complexity levels, slightly reduced risk levels on average.
% We can see that FCOGB has typically strongly reduced risk levels on average.
% , and on par or slightly increased risk levels in the worst case---with the exception of the comparison to the gradient sum variant, where the risk increases in the worst case appear more pronounced.
% However, even in this comparison FCOGB appears to have the more substantial advantage: In the best case complexity it outperforms Gradient Sum by more than 10 percentage points normalized risk in 44\% of the datasets. Conversely, at the worst case level, it is only outperformed by this margin in 9\% of the datasets.
Performing one-sided paired t-tests at significance level 0.05 (with Bonferroni correction for 8 hypotheses) reveals that FCOGB significantly outperforms all other variants with a margin of at least 0.001 average normalized training risk (while there is no significant winner in terms of test risk---likely due to a lack of regularization for larger ensemble sizes). 
%(ii) FCOGB significantly outperforms gradient boosting and the gradient sum variant by the same margin in terms of the average risk difference. Extreme gradient boosting is also outperformed significantly, however, counter-intuitively only after excluding its extremely weak performances on the counting problems (accounted for in the Bonferroni correction, although as a post-hoc consideration), which otherwise let the standard deviation explode.
%where it is worthwhile to note that the reason that the average difference is not significant for extreme gradient boosting is the latter's extremely weak performance on some counting problems, which let the standard deviation of the sample explode. 
% (iii) For the worst-case level, FCOGB is only significantly outperformed by the gradient sum approach. While these results refer to the training error, the test error show similar trends, albeit with higher variance, which causes the average performance comparisons to only be significant without Bonferroni correction.

% Table \ref{tb:comparison} shows the experiment results for several benchmark datasets of classification, regression and Poisson regression problems using gradient boosting, XGBoost and FCOGB. 
% For all datasets, the FCOGB algorithm produces additive rule ensembles which have smaller risk values than the other two. 
% The average risks of the models with cognitive complexity 30 generated by FCOGB is shown in the table, as well as the average advantage of the risks of FCOGB over the other two at the same cognitive level.

% In addition, the best case and the worst case difference from the models by FCOGB to the other two algorithms are shown in the table, as well as the cognitive complexity where these differences are obtained. The best case differences between the risks of models generated by FCOGB and XGBoost are more than 1 for 4 datasets of Poisson regression problems. The reason is that XGBoost cannot handle Poisson regression problems well.

% In addition to these overall comparisons, it is also interesting to investigate which of the components FCOGB carry what weight in outperforming in particular the most closely related standard gradient boosting function. To this end, the right-hand side of Fig.~\ref{fig:ablation_study} shows the result of an ablation study where standard gradient boosting is first modified by weight-correction, then by the advanced objective function, and then by upgrading greedy to branch-and-bound search.
% As can be seen, the overall advantages are building up through the individual steps, which contribute roughly equally to the performance gains.

% FCOGB algorithm is a variant of gradient boosting which involves a fully-correction step, orthogonal projection and optimal branch-and-bound search. 
% To show the benefits we get from gradient boosting to FCOGB in each step of modification, the first three sub-figures in Figure \ref{fig:ablation_study} compare gradient boosting, fully-corrective boosting without orthogonal projection, FCOGB with greedy search and FCOGB with optimal search.
% Each figure shows the worst case and best case risk difference of the compared algorithms. 

% The first three columns in Figure \ref{fig:ablation_study} also show the overall comparison of FCOGB with gradient sum, gradient boosting and XGBoost. each point in the figure shows the two risk values when the best case or worst case differences of risk values are achieved.

% As the results show, FCOGB has obvious advantages over gradient boosting and XGBoost for all the three types of problems in terms of the tradeoff between accuracy and cognitive complexity. 
% Although in some cases, gradient boosting and XGBoost has lower risk values than FCOGB, usually their differences are not compatible with the advantages of FCOGB over the other two algorithms.


\begin{figure*}[t!]
\vskip 0.1in
\begin{center}
% \begin{subfigure}
% \centering
\includegraphics[width=0.57\columnwidth]{Images/coverage.pdf}
% \end{subfigure}
% \begin{subfigure}
% \centering
\includegraphics[width=0.40\columnwidth]{Images/combined_time_comp.pdf}
\label{fig:time_tic}
% \end{subfigure}
% \begin{subfigure}
% \centering
% \includegraphics[width=0.20\columnwidth]{Images/diabete_time_comp2.pdf}
% \label{fig:time_diab}
% \end{subfigure}
\vskip -0.1in
\caption{First three: the comparison of the coverage rate of Gradient Boosting, XGBoost, Gradient Sum and FCOGB. The upper (resp. lower) half of the green line means the coverage rate of FCOGB is higher (resp. lower) than the other method. Last two: the comparison of the running time of Gradient boosting, XGBoost and FCOGB for the benchmark datasets \texttt{breast cancer} and \texttt{diabetes} of generating rule ensembles with cognitive complexity 50.}
\label{fig:compare_coverage}
\end{center}
\vskip -0.3in
\end{figure*}
\paragraph{Coverage}
To compare the generality of the rules learned by the new objective function in comparison to the existing ones, we performed an additional experiment where we first used one of the previous objective functions to generate rule ensembles with ten rules for all datasets.
Then for each partial rule ensemble, we applied the orthogonal gradient boosting objective function to find an alternative rule. Importantly, we used branch-and-bound with admissible bounding functions for all the alternative objectives to avoid confounding through sub-optimal greedy solutions.
In Fig.~\ref{fig:compare_coverage} we compare the relative coverage, i.e., the relative number of selected data points $\|\q\|^2/n$, of the rules discovered by the original algorithms to the ones discovered by FCOGB.
% We define the coverage rate as the ratio of the number of data points covered by the neyw rule and the total number of data points:
% \begin{equation}
%     \text{CR} = \frac{|I(q)|}{n},
% \end{equation}
% where $I(q)$ is the support set of the query $q$, and $n$ is the total number of data points. 
% We firstly use one of gradient sum, gradient boosting, XGBoost and FCOGB to build rule ensembles of rule numbers from 1 to 10. Based on the same ensembles, we run gradient sum, gradient boosting, XGBoost and FCOGB to generate one more new rule to add into the ensemble to compare the coverage rate of the newly generated rule. 
% Figure \ref{fig:compare_coverage} shows the comparison of the coverage rate of these four algorithms.
% It can be seen that the FCOGB algorithm generates rules which cover more data points than the other algorithms in most cases. 
The outcome is that 81.1\% of the FCOGB rules covers more data points than gradient boosting, and similarly 71.3\% of its rules cover more data points than those generated by XGBoost. In contrast, only 47.2\% of the FCOGB rules cover more datapoint than the ones discovered by gradient sum.
%There are 7.6\% of the FCOGB rules covering more than 50\% data points while the rules generated by gradient boosting cover less than 50\%, and this number is 6.0\% for gradient boosting and 6.1\% for gradient sum. 
These results are in alignment with the theoretical expectation in terms of the influence of the coverage on the objective values where gradient sum is completely unaffected, whereas orthogonal gradient boosting has a denominator that tends to grow with coverage albeit less than the one of gradient boosting.
%The number of data points covered by rules generated by FCOGB and gradient sum approach are similar to each other. This is because the gradient sum approach tends to select rules which cover more data points. 

\paragraph{Computation time}
% \begin{figure}
% \vskip 0.1in
% \begin{center}
% \begin{subfigure}
% \centering
% \includegraphics[width=0.48\columnwidth]{Images/breast_time.pdf}
% \label{fig:time_tic}
% \end{subfigure}
% \begin{subfigure}
% \centering
% \includegraphics[width=0.46\columnwidth]{Images/diabete_time.pdf}
% \label{fig:time_diab}
% \end{subfigure}
% \end{center}
% \vskip -0.1in
% \caption{Comparison of the running time of Gradient boosting, XGBoost and FCOGB for the benchmark datasets \texttt{breast cancer} and \texttt{diabetes} of generating 10 rules.}
% \label{fig:time_comp}
% \end{figure}
We also compare the computational cost of generating rule ensembles with cognitive complexity 50 by different algorithms in Tab \ref{tb:comparison}.
Comparing the computational cost of FCOGB to XGB, the other algorithm utilizing the more expensive branch-and-bound search, the costs are in the same order of magnitude except for one extreme case (wine) where FCOGB is a factor of 26 slower.
% Comparing to the two greedy variants, FCOGB is still faster than gradient boosting for 13 datasets, and faster than the gradient sum approach for 5 datasets.
Comparing to the two greedy variants, FCOGB is in the same order of magnitude as gradient boosting for most datasets. Unsuprisingly, there are a few examples where greedy search vastly outperforms branch-and-bound, in one case (telco churn) by a factor of around 76.
However, overall, the results confirm that branch-and-bound search is a practical algorithm in absolute terms: For 23 benchmark dataset, FCOGB is able to finish training a model of cognitive complexity of 50 within one minute. Most of the  other experiments run within 15 minutes except one dataset (telco churn) which require longer running time.  
% The last 4 columns in Table \ref{tb:comparison} show the computation time of gradient sum, gradient boosting, XGBoost and FCOGB for generating 10 rules. 
% Totally, FCOGB is able to finish training a model of 10 rules within 1 minute for 25 benchmark datasets. Most of the experiments can be finished within 5 minutes except 2 datasets (telco churn and mobile prices) which require longer running time. 
% Among all the 34 benchmark datasets, there are 24 datasets where FCOGB outperforms XGBoost. For the other 10 datasets, the running time of FCOGB is no more than 4 times of that of XGBoost except one dataset where XGBoost is much faster than FCOGB (Wine). 
% Generally, FCOGB use more time than the gradient sum approach and gradient boosting, as these two algorithms are using greedy search instead of branch-and-bound.
% FCOGB is faster than gradient boosting for 13 datasets, and FCOGB performs better than the gradient sum approach for 5 datasets.
% When comparing with the gradient sum algorithm, the running time of FCOGB is within a factor of 5 of the time of gradient sum for 23 datasets. There are 8 datasets where FCOGB uses more than 5 times of the computation times of gradient sum. Furthermore, for 3 datasets, the time required by FCOGB is 50 times of the running time of gradient sum.
Finally, Fig.~\ref{fig:compare_coverage} shows the detailed computation time of all algorithms in terms of cognitive complexity, including the naive implementation of FCOGB for \textit{breast cancer} and \textit{diabetes}, which 
shows that the performance improvement through Thm.~\ref{thm:fast_prefix} is critical to bring the computational complexity on par with XGB. 




==> rebuttal_table.tex <==
\begin{table}[]
\caption{Comparison of normalised training risks and computation times for rule ensembles, averaged over cognitive complexities between 1 and 50, using SIRUS(SRS), Gradient Sum(GS), Gradient boosting (GB), XGBoost (XGB) and FCOGB, for benchmark datasets}
\begin{footnotesize}
\begin{center}
\begin{tabular}{l@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}c@{\hskip 0.03in}}
\toprule
 &  &  & \multicolumn{5}{c}{Training Risks} & \multicolumn{5}{c}{Testing Risks} \\
\multirow{-2}{*}{Dataset} & \multirow{-2}{*}{$d$} & \multirow{-2}{*}{$n$} & SRS & GS & GB & XGB & FCOGB & SRS & GS & GB & XGB & FCOGB\\ 
\hline
titanic & 7 & 1043 & .895 & .653 & .656 & .646 & \textbf{.621} & .894 & .695 & .707 & .711 & \textbf{.695} \\
tic-tac-toe & 27 & 958 & .892 & .757 & .641 & .621 & \textbf{.604} & .885 & .809 & .682 & .605 & \textbf{.586} \\
iris & 4 & 150 & .685 & .239 & .248 & .329 & \textbf{.232} & .745 & .521 & .440 & .459 & \textbf{.424} \\
breast & 30 & 569 & .569 & .277 & .310 & .314 & \textbf{.239} & .627 & \textbf{.269} & .362 & .338 & .342 \\
wine & 13 & 178 & .578 & .198 & .223 & .192 & \textbf{.183} & .621 & .341 & .443 & .409 & \textbf{.250} \\
ibm hr & 32 & 1470 & .980 & .567 & \textbf{.555} & .569 & .564 & .974 & .640 & .666 & .630 & \textbf{.617} \\
telco churn & 18 & 7043 & .944 & .679 & .683 & .678 & \textbf{.667} & .945 & .663 & .677 & .665 & \textbf{.653} \\
gender & 20 & 3168 & .566 & .250 & .254 & .271 & \textbf{.247} & .570 & \textbf{.264} & .267 & .285 & .265 \\
banknote & 4 & 1372 & .854 & .305 & .267 & .290 & \textbf{.228} & .858 & .312 & .268 & .299 & \textbf{.229} \\
liver & 6 & 345 & .908 & .809 & \textbf{.805} & .811 & .830 & .917 & .909 & .901 & \textbf{.878} & .881 \\
magic & 10 & 19020 & .906 & .719 & .709 & .710 & \textbf{.707} & .903 & .700 & .693 & .693 & \textbf{.687} \\
adult & 11 & 30162 & .804 & .604 & .609 & .604 & \textbf{.559} & .802 & .612 & .623 & .615 & \textbf{.573} \\
digits5 & 64 & 3915 & \textbf{.248} & .355 & .331 & .354 & .337 & \textbf{.262} & .347 & .328 & .348 & .331 \\ \hline
insurance & 6 & 1338 & .169 & .130 & .142 & .144 & \textbf{.127} & .177 & .132 & .145 & .147 & \textbf{.131} \\
friedman1 & 10 & 2000 & .180 & .051 & .052 & .051 & \textbf{.019} & .165 & .054 & .057 & .059 & \textbf{.022} \\
friedman2 & 4 & 10000 & .082 & .069 & .064 & .059 & \textbf{.023} & .082 & .071 & .065 & .060 & \textbf{.023} \\
friedman3 & 4 & 5000 & .093 & .026 & .022 & .022 & \textbf{.009} & .092 & .029 & .027 & .027 & \textbf{.011} \\
wage & 5 & 1379 & .427 & .370 & .361 & .356 & \textbf{.351} & \textbf{.341} & .358 & .406 & .367 & .375 \\
demographics & 13 & 6876 & .219 & .214 & .214 & .214 & \textbf{.212} & \textbf{.209} & .216 & .217 & .217 & .215 \\
gdp & 1 & 35 & .063 & .020 & .020 & .020 & \textbf{.020} & .059 & .020 & .020 & .020 & \textbf{.020} \\
used cars & 4 & 1770 & .373 & \textbf{.130} & .205 & .153 & .132 & .427 & .101 & .157 & .100 & \textbf{.082} \\
diabetes & 10 & 442 & .156 & .138 & .141 & .139 & \textbf{.132} & .188 & \textbf{.140} & .142 & .147 & .148 \\
boston & 13 & 506 & .101 & .088 & .086 & .086 & \textbf{.082} & .105 & \textbf{.081} & .086 & .087 & .088 \\
happiness & 8 & 315 & .109 & .030 & .031 & .030 & \textbf{.030} & .109 & \textbf{.033} & .038 & .038 & .036 \\
life expect. & 21 & 1649 & .109 & .026 & .026 & .026 & \textbf{.025} & .110 & .027 & .027 & .027 & \textbf{.026} \\
mobile prices & 20 & 2000 & .148 & \textbf{.131} & .137 & .137 & .134 & .140 & \textbf{.134} & .143 & .145 & .139 \\
suicide rate & 5 & 27820 & .547 & .566 & .561 & .561 & \textbf{.531} & .514 & .544 & .542 & .542 & \textbf{.509} \\
videogame & 6 & 16327 & \textbf{.895} & .953 & .953 & .953 & .953 & .850 & \textbf{.720} & \textbf{.720} & \textbf{.720} & \textbf{.720} \\
red wine & 11 & 1599 & .072 & .034 & .035 & .034 & \textbf{.034} & .073 & \textbf{.035} & .036 & .036 & \textbf{.035} \\ \hline
covid vic & 4 & 85 & NA & .153 & .121 & .132 & \textbf{.105} & NA & .182 & \textbf{.100} & .133 & .104 \\
covid & 2 & 225 & NA & .344 & .371 & .891 & \textbf{.335} & NA & .459 & .411 & .741 & \textbf{.407} \\
bicycle & 4 & 122 & NA & .317 & .324 & .337 & \textbf{.295} & NA & .366 & .478 & .457 & \textbf{.328} \\
ships & 4 & 34 & NA & \textbf{.174} & .181 & 1.927 & .186 & NA & .197 & .203 & 4.156 & \textbf{.172} \\
smoking & 2 & 36 & NA & .127 & .128 & .163 & \textbf{.091} & NA & .136 & .250 & .322 & \textbf{.103}\\
\bottomrule
\end{tabular}
\end{center}
\end{footnotesize}
\end{table}
